Quantitative Regular Expressions for Arrhythmia Detection Algorithms

Motivated by the problem of verifying the correctness of arrhythmia-detection algorithms, we present a formalization of these algorithms in the language of Quantitative Regular Expressions. QREs are a flexible formal language for specifying complex numerical queries over data streams, with provable runtime and memory consumption guarantees. The medical-device algorithms of interest include peak detection (where a peak in a cardiac signal indicates a heartbeat) and various discriminators, each of which uses a feature of the cardiac signal to distinguish fatal from non-fatal arrhythmias. Expressing these algorithms' desired output in current temporal logics, and implementing them via monitor synthesis, is cumbersome, error-prone, computationally expensive, and sometimes infeasible. In contrast, we show that a range of peak detectors (in both the time and wavelet domains) and various discriminators at the heart of today's arrhythmia-detection devices are easily expressible in QREs. The fact that one formalism (QREs) is used to describe the desired end-to-end operation of an arrhythmia detector opens the way to formal analysis and rigorous testing of these detectors' correctness and performance. Such analysis could alleviate the regulatory burden on device developers when modifying their algorithms. The performance of the peak-detection QREs is demonstrated by running them on real patient data, on which they yield results on par with those provided by a cardiologist.

==> camera - Copy - Copy (2)/chapters/abstract.tex <==
\begin{abstract}
Motivated by the problem of verifying the correctness of arrhythmia-detection algorithms, we present a formalization of these algorithms in the language of \textit{Quantitative Regular Expressions}. 
QREs are a flexible formal language for specifying complex numerical queries over data streams, with provable runtime and memory consumption guarantees.
The medical-device algorithms of interest include \textit{peak detection} (where a peak in a cardiac signal indicates a heartbeat) and various \textit{discriminators}, each of which uses a feature of the cardiac signal to distinguish fatal from non-fatal arrhythmias.
Expressing these algorithms' desired output in current temporal logics, and implementing them via monitor synthesis, is cumbersome, error-prone, computationally expensive, and sometimes infeasible. 

In contrast, we show that a range of peak detectors (in both the time and wavelet domains) and various discriminators at the heart of today's arrhythmia-detection devices are easily expressible in QREs.
The fact that one formalism (QREs) is used to describe the desired end-to-end operation of an arrhythmia detector opens the way to formal analysis and rigorous testing of these detectors' correctness and performance. 
Such analysis 
could alleviate the regulatory burden on device developers when modifying their algorithms.
The performance of the peak-detection QREs is demonstrated by running them on real patient data, on which they yield results on par with those provided by a cardiologist.
\keywords{Peak Detection; Electrocardiograms; Arrythmia Discrimination; ICDs; Quantitative Regular Expressions}
\end{abstract}


==> camera - Copy - Copy (2)/chapters/acknowledgments.tex <==
\section*{Acknowledgments}
The authors would like to thank Konstantinos Mamouras for insightful discussions about QREs and for providing the QRE Java library we used in this paper.  This work is supported in part by %
AFOSR Grant FA9550-14-1-0261 % ARRIVE
and NSF Grants
IIS-1447549, % CR and smolka: Big Data 
CNS-1446832, % smolka and grosu: Compositional, Approximate, and Quantitative Reasoning for Medical Cyber-Physical Systems
CNS-1446664, % Houssam:  Compositional, Approximate, and Quantitative Reasoning for Medical Cyber-Physical Systems
CNS-1445770, % smolka: FDA SIR
and CNS-1445770. % smolka: CPS Medical Device Workshop
E.B.\ and R.G.\ acknowledge the partial support of the Austrian National Research Network  S 11405-N23 and S 11412-N23 (RiSE/SHiNE) of the Austrian Science Fund (FWF) and the ICT COST Action IC1402 Runtime Verification beyond Monitoring (ARVI).
%Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of these organizations.


The authors would like to thank Konstantinos Mamouras for insightful discussions about QREs and for providing the QRE Java library we used in this paper.  This work is supported in part by 
AFOSR Grant FA9550-14-1-0261 
and NSF Grants
IIS-1447549,
CNS-1446832,
CNS-1446664,
CNS-1445770,
and CNS-1445770.
E.B.\ and R.G.\ acknowledge the partial support of the Austrian National Research Network  S 11405-N23 and S 11412-N23 (RiSE/SHiNE) of the Austrian Science Fund (FWF) and the ICT COST Action IC1402 Runtime Verification beyond Monitoring (ARVI).


The authors would like to thank Konstantinos Mamouras for insightful discussions about QREs and for providing the QRE Java library we used in this paper. This work is supported in part by %
AFOSR Grant FA9550-14-1-0261
and NSF Grants
IIS-1447549,
CNS-1446832, 
CNS-1446664, 
CNS-1445770, 
and CNS-1445770, 
and Austrian National Research Network grants 
S 11405-N23 and S 11412-N23 (RiSE/SHiNE of the FWF) and the ICT COST Action IC1402 Runtime Verification beyond Monitoring.

==> camera - Copy - Copy (2)/chapters/algosForPeakDetection.tex <==
\section{Implementing a commercial peak detector as a QRE}
\label{sec:mdt pda}
We now provide a \ac{QRE} implementation of the \ac{PDA} found in some \ac{ICD} models of Medtronic, a major medical devices manufacturer.
This example illustrates two important points about the use of \acp{QRE}:  
the first is that, to target certain applications without violating the constraints of regular parsing, we may need to use a richer set of operations $\opset$ (thus moving some of the complexity of the specification into the operations). 
This is certainly allowed by the current theory of \acp{QRE}, but then one must carefully analyze the resulting evaluation complexity since richer operations will, a priori, require more memory and time. 
In other words, we feel free to enlarge the set of operations without departing from the \ac{QRE} philosophy of being a declarative programming language that allows a global view of the data stream and minimal maintenance of state on the part of the programmer.
The second point this example illustrates is that the streaming setup is useful independently of the basic matching process. 
I.e. whether substreams are matched to regular expressions or, say, bounded temporal logic formulas, the streaming setup and the regular combinators are useful in thinking about the problems we face.

%\begin{figure}[t]
%	\centering
%\includegraphics[scale=0.2]{figures/placeHolder}
%\caption{Peak detection based on a varying threshold as performed in Medtronic devices.}
%\label{fig:mdt pda}
%\end{figure}

\subsection{Natural language description of the peak detector}
The \ac{PDA} defines peaks as points where the signal $y(t) = |\egm(t)|$, which equals the absolute value of the electrogram $\egm(t)$, exceeds a time-varying threshold $p(t)$.
%See Fig. \ref{fig:mdt pda}.
When this happens, a \emph{blanking period} of pre-fixed duration $BL$ is entered. 
In what follows we measure $BL$ in numbers of samples since the sampling rate is uniform.
During the blanking period, no events are recorded, regardless of the relation between threshold and signal.
Also during the blanking period, the maximum value of the signal is recorded.
Let $y(t_m)$ be the value of the maximum, and $t_m$ its time.
At the end of the blanking period, the threshold is reset to the value $0.75 y(t_m)$. 
From there, the threshold decreases exponentially at a pre-specified decay rate $\lambda$.
I.e., after the blanking period, the threshold obeys $p(t) = 0.75y(t_m)e^{-\lambda (t-t_m -BL)}$.
The decay in threshold continues until either a new event is detected, or a minimum threshold value $\underline{p}$ is reached. 
If the minimum threshold value is reached, the threshold remains there until an event is detected.

\subsection{The \ac{QRE}}
\label{sec:mdt pda qre}
The data stream consists of successive uniformly sampled values of $y \in D = \reals$, and the cost domain is $C = \reals$.
The output stream will be a string of time instants when a peak occurred.\footnote{Strictly speaking, the output is a single cost term which is the value of the QRE on the input stream. But stream composition allows us to produce output streams that are then passed along to other QREs.}
If the evolving threshold $p(t)$ were given as part of the input stream\footnote{I.e.. if the data item were $d = (y,p) \in \reals^2$.}, then the above algorithm is easily implemented by concatenating thee QREs: 
the first would iteratively match $y < p$, i.e. $r_1 = (y < p)^*$ ($r_1$ is the RE of the first QRE, etc).
The second would match the signal exceeding the threshold: $r_2 = y \geq p$.
And the third would match the blanking period: $r_3 = D^L$, where $L$ is the blanking duration.
Finally we iterate:
\begin{equation}
r_{mdt1} = (r_1 \cdot r_2 \cdot r_3)^* = ((y<p)^*(y\geq p)D^L)^*
\end{equation}

To produce the time instant at which the peak occurred, the corresponding QRE $mdt1$ only needs to use the sum operation.
Computing the threshold $p$ from the stream $y_1\ldots y_n \in \reals^*$ on the other hand requires a more powerful operation.
The threshold is now treated as a parameter that is updated by the \ac{QRE}. 
Intuitively, with each new voltage value, either the threshold is decreased (in case $y < p$),  or a blanking period is entered (), or a blanking counter is increased (in case $y \geq p$ or the algorithm is already in the blanking period) or the threshold is reset (in case the blanking period expires). 
Because the basic predicates $\phi$ of a symbolic \ac{RE} do not allow to compare a data item $y$ to a parameter value $p$ we need to implement the threshold evolution in an $op$, which we will call $ThEv$.
The implementation details are simple and we omit them for the sake of space.
The peak-detection \ac{QRE} is then simply an iteration of $ThEv$:
\begin{equation}
\label{eq:mdt ThEv}
mdt2 = \iter{ThEv}(d \in \reals?d)
\end{equation}
It is easy to verify that $ThEv$ requires time and memory that are independent of the length of the input string since they only need to consider the current value of the voltage (and internal variables). 
Moreover note that the only basic predicate being used is $d \in \reals$, which takes constant time (in fact, since the data domain is assumed to be $\reals$ no actual check takes place). 
Therefore, despite using a more `powerful' operation, it holds that the evaluator $M_{mdt2}$ processes each data item in time $poly(|mdt2|)$, independently of the length of the string.

\subsection{Experiments}
\label{sec:ex mdt pda}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figures/A177VT2vfiltD1L2Init200BL150}
\caption{\small Rectified EGM of a \ac{VF} showing the peaks detected by QRE $mdt2$ as red circles. By design of this PDA, the circles don't coincide with the actual peaks but precede them by a bit. This doesn't affect the \ac{ICD} operation. }
\label{fig:A177VT2vfiltD1L2Init200BL150}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{figures/A176VT1vfiltD1L2Init300BL80}
	\caption{\small Rectified EGM of a \ac{VT} showing the peaks detected by QRE $mdt2$ as red circles.}
	\label{fig:A176VT1vfiltD1L2Init300BL80}
\end{figure}

We implemented the \ac{QRE} of Eq. \eqref{eq:mdt ThEv}. 
In Fig. \ref{fig:A177VT2vfiltD1L2Init200BL150} we show the results of running it on a \acf{VF} \acf{EGM} collected from a patient during an electrophysiology study.
Note the varying amplitude typical of VF and which is challenging to peak detectors. 
Some peaks are double-counted (e.g. around time 3500) which leads to over-counting and potentially to inappropriate therapy as the heart rate is over-estimated.
Fig. \ref{fig:A176VT1vfiltD1L2Init300BL80} shows $mdt2$ running on a \acf{VT} \ac{EGM}. 
Because \ac{VT} is more organized than a \ac{VF} the \ac{PDA} makes fewer mistakes (in fact, none in this case). 
 
%\input{mdtCLTLformula}

%Given the input string of voltage values, we want to repeatedly extract a substring where the signal is below the threshold (and the threshold is being decreased) followed by a substring where the signal exceeds the threshold (and the blanking period is in effect). 
%I.e. we want to iteratively match the following pattern in the signal:
%\[(y < p? \text{ decrease threshold })^* (y \geq p? \text{ blanking period})\]
%
%First, we describe the threshold decrease. 
%Let $p$ be a parameter holding the value of the threshold, and let $\underline{p} \in \reals$ be the constant that equals the minimum threshold. 
%Then:
%\[decThreshold = iter[p\rangle(y<p? \max(\underline{p}, pe^{-\lambda \Delta t}))\]
%$decThreshold$ matches any strings where the data item $y$ is always below the (decaying) threshold.
%It is of the form QRE($\reals^*, \{p\},\reals$).
%
%Next, the blanking period is conveniently expressed as
%\[blank = (y \geq p?y) \splitp{p} \iter{max}_{BL}(y \in \reals? 0.75y)\]
%This matches a length-$(BL+1)$ string, whose first element exceeds or equals the threshold $p$.
%It evaluates to 0.75 the maximum value of the signal in a window of size $BL$.
%It is of the form QRE($\reals^{BL+1}, \{p\},\reals$).
%
%Since $decThreshold$ and $beat$ are unambiguously concatenatable, we may write
%\[beat = decThreshold \splitp{p} blank\]
%
%Unfortunately, $beat$ is not unambiguously iterable: a string can iteratively match $\reals^*\reals^{BL+1}$ in more than one way.



==> camera - Copy - Copy (2)/chapters/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We have demonstrated that peak detection, a common and essential signal processing task, cannot be specified in temporal (or time-frequency) logic.
We leveraged a characterization of peaks as singularities in the wavelet domain, formalized it using \acfp{QRE}, and demonstrated its performance on real patient electrograms.
In other work, we use this peak characterization in order to specify various arrhythmia discriminators of ICDs in QREs. 
Finally, it would be very interesting to consider what kind of compile- or run-time analysis questions (e.g., refinement, prediction, and control) can be answered for \acp{QRE} in the specific context of \ac{ICD} verification.


==> camera - Copy - Copy (2)/chapters/differentLogics.tex <==
\section{Challenges in Formalizing ICD Discrimination and Peak Detection}
\label{sec:manylogics}

%%\todo[inline]{In~\cite{BrimDSV14} the authors show that the
%monitoring algorithm for STL with nesting freeze 
%quantifiers is polynomial in the number of intervals on 
%which the signals is defined and the size of the syntactic 
%tree of the formula, but it is exponential in the number 
%of the nested freeze operators in the formula.}

% we consider three funamenatl discrimination  and PD tasks common to all arrh. dics algos.

This section demonstrates the difficulties that arise when using temporal logic to express the discrimination and peak-detection tasks common to all arrhythmia-detection algorithms.
Specifically: different discriminators require the use of different logics, whose expressive powers are not always comparable; 
the formulas quickly become unwieldy and error-prone;
and the complexity of the monitor-synthesis algorithm, \textit{when} it is available, rapidly increases due to nesting of freeze quantification.
On the other hand, it will be shown that \acp{QRE} are well-suited to these challenges: 
all tasks are expressible in the \ac{QRE} formalism,
the resulting expressions are simple direct encodings of the tasks, 
and their monitors are efficient.
The syntax and semantics of the logics will be introduced informally as they are outside the scope of this paper.

An ICD \textit{discriminator} takes in a finite discrete-timed signal $w: \{0,\ldots,T\} \rightarrow D$.
%Unless otherwise noted, the range $D$ is $\{0,1\}$ where a 1 indicates a heartbeat, and a 0 the absence thereof.
%We will sometimes treat $w$ as a finite string in $D^*$, and this should cause no confusion.
(Signal $w$ will also sometimes be treated as a finite string in $D^*$ without causing confusion).
The discriminator processes the signal $w$ in a sliding-window fashion. 
When the window is centered at time instant $t$, the discriminator computes some feature of the signal (e.g., the average heart rate) and uses this feature to determine if the rhythm displays a potentially fatal arrhythmia in the current window (at time $t$).
The ICD's overall Fatal vs Non-Fatal decision is made by combining the decisions from all discriminators.

In what follows, several discriminators that are found in the devices of major ICD manufacturers are described.
Then for each discriminator, after discussing the challenges that arise in specifying the discriminator in temporal logic, a \ac{QRE} is given that directly implements the discriminator.
This will also serve as a soft introduction to \ac{QRE} syntax.
Fix a data domain $D$ and a cost domain $C$.
For now, we simplify things by viewing a QRE $\qre{f}$ as a regular expression $r$ along with a way to assign costs to strings $w \in D^*$.
If the string $w$ matches the regular expression $r$, then the QRE maps it to $\qre{f}(w) \in C$.
If the string does not match, it is mapped to the undefined value $\bot$.
The QRE's computations can use a fixed but arbitrary set of \textit{operations} (e.g., addition, max, or insertion into a set).
Operations can be thought of as arbitrary pieces of code.

%
The first example of discriminator checks whether the number of heartbeats in a one-minute time interval is between 120 and 150.
This requires the use of a counting modality like that used in CTMTL~\cite{Krishna16_CountingMTL}. 
If $p$ denotes a heartbeat, then the following CTMTL formula evaluates to true exactly when the number of heartbeats lies in the desired range: $\text{C}_{[0,59]}^{\geq 120}p\,\wedge\,\text{C}_{[0, 59]}^{\leq 150}p$.
%\begin{equation*}
%\text{C}_{[0,59]}^{\geq 
%	120}p\,\wedge\,\text{C}_{[0, 59]}^{\leq 
%	150}p
%\end{equation*} 

This is equally easily expressed as a \ac{QRE}: match $60$ signal samples (at a 1Hz sampling rate), and at every sample where $p$ is true (this is a heartbeat), add 1 to the cost, otherwise add 0. Finally, check if the sum is in the range:
\begin{equation*}
\mathtt{inrange}(iter_{60}\!-\!add(p?1\textrm{ else } 0))
\end{equation*}

The second discriminator determines whether the heart rate increases by at
least 20\% when measured over consecutive and disjoint windows of 4~beats.
In logic, this requires explicit clocks, such as those used in Explicit Clock Temporal Logic XCTL~\cite{Harel90_XCTL}, since the
beat-to-beat delay is variable. 
So let $T$ denote the time state (which keeps track of time) and let the $x_i$'s be rigid clock variables that store the times at which $p$ becomes true.
The following XCTL formula expresses the desired discriminator:
\begin{align*}
\always(p\,\wedge (x_1=T)\,\wedge\, \eventually(
p\,\wedge \ldots \eventually
(p\,\wedge\, (x_9=T)\,
\wedge\,[(x_5-x_1)\cdot 0.8 \geq x_9-x_5] )\ldots) )
\end{align*}
Note the need to explicitly mark the 9 heartbeats and nest the setting of clock variables 9-deep.
This computation can be described in a \ac{QRE} in a simpler, more concise manner.
Just like the usual regular expressions, simpler \acp{QRE} can be combined into more complex ones. 
We will now use the $\splitop{op}$ combinator (see Fig.~\ref{fig:qre illustrations}): given the input string $w = w_1w_2$ which is a concatenation of strings $w_1$ and $w_2$, and \acp{QRE} $\qre{f},\qre{g}$, $\splitop{op}(\qre{f},\qre{g})$ maps $w$ to the cost value $op(\qre{f}(w_1), \qre{g}(w_2))$, where $op$ is some operator (e.g., averaging).
So let \ac{QRE} $\qre{fourBeats}$ match four consecutive beats in the boolean signal $w$ and let it compute the average cycle length of these 4 beats. Let $inc(x,y)$ be an operation that returns True whenever $0.8x \geq y$.
Then \ac{QRE} $\qre{suddenOnset}$ does the job:
\begin{align*}
\qre{suddenOnset}\,&:=&\,\splitop{inc}(\qre{fourBeats},\,\qre{fourBeats}) 
\\
\qre{fourBeats} &:=& iter_4\!-\!avg(\qre{intervalLength})
\\
\qre{intervalLength} &:=& \splitop{left}(\qre{countzeros}, 1)  \quad /\!/\, left(a,b) \textrm{ returns } a
\end{align*}

The third discriminator takes in a three-vaued signal $w:\Ne \rightarrow \{0,A,V\}$ where a 0 indicates no beat, an $A$ indicates an atrial beat, and a $V$ indicates a ventricular beat.
One \textit{simplified} version of this discriminator detects whether this pattern occurs in the current window: $V 0^{a:b} A 0^{c:d} V 0^{e:f} A 0^{g:h} V$.
Here, $a$ and $b$ are integers, and $0^{a:b}$ indicates between $a$ and $b$ repetitions of 0. 
This can be expressed in discrete-time Metric Temporal Logic~\cite{Koymans90}. 
E.g. the prefix $V 0^{a:b}A$ can be written as
$w=V \implies X ((w=0)\, \until_{[a+1,b]}(w=A))$.
And so on.
This quickly becomes unwieldy as the pattern itself becomes lengthier and with more restrictions on the timing of the repetitions.
On the other hand, this is trivially expressed as a (quantitative) regular expresssion.

Our final example comes from Peak Detection (PD), which takes in a real-valued signal $v:\Ne \rightarrow \Re_{\geq 0}$.
For \textit{one component} of this PD, the objective is to detect when $v(t)$ exceeds a threshold value $h >0 $ which
is reset as a function of the previous peak value.
Thus the logic must remember the value of that peak.  
This necessitates \emph{freeze quantification} of state variables, as used in
Constraint LTL with Freeze Quantification $\CLTLF$~\cite{DEMRI07_ConstraintLTL} ($\freeze_{z=v}$ means that we freeze the variable $z$ to the value of $v$):
\begin{eqnarray*}
	\always (v > h \implies \freeze_{BL=1} \eventually  \left( 
	\formula_{\text{local-max}} \implies  h = 0.8z_2 \right))
	\\
	\formula_{\text{local-max}} \defeq  \freeze_{z_1=v} \nxt 
	(\freeze_{z_2=v} \nxt (z_2 > z_1 \land z_2> v))
\end{eqnarray*}	
The nesting of freeze quantifiers increases the chances of making errors when writing the specification and decreases its legibility.
More generally, monitoring of nested freeze quantifiers complicates the monitors significantly and increases their runtimes. 
E.g., in~\cite{BrimDSV14} the authors show that the
monitoring algorithm for STL with nested freeze 
quantifiers 
%is polynomial in the number of intervals on which the signal is defined and the size of the syntactic tree of the formula, but it 
is exponential in the number 
of the nested freeze operators in the formula.
This becomes more significant when dealing with the \textit{full} PD, of which the above is one piece.
On the other hand, we have implemented an even more complex PD as a QRE (Section~\ref{sec:qre_wpm}).

The reader will recognize that the operations performed in these tasks are quite common, like averaging, variability, and state-dependent resetting of values, and can conceivably be used in numerous other applications.

This variety of logics required for these tasks, all of which
are fundamental building blocks of ICD operation, means that a temporal logic-based approach to the problem is unlikely to yield a unifying view, whereas QREs clearly do. 
In the rest of the paper, the focus is placed on peak detection, as it is more complicated than discrimination, and offers a strong argument for the versatility and power of \acp{QRE} in medical-device algorithms.

==> camera - Copy - Copy (2)/chapters/discrimination.tex <==
\section{Arrhythmia Discrimination and Experimental Results}
\label{sec:discrimination}
In Section \ref{sec:many logics} we illustrated the difficulty of using temporal logics 
We briefly illustrate how the discrimination tasks outlined in Section \ref{sec:many logics} can be easily and clearly implemented as QREs.
In this section, we will briefly illustrate how different logics are 
needed for different discriminators, thus prompting the use of 
\acp{QRE}.
%
For example, to
express that the number of heartbeats in a one minute interval must 
be between 90 and 120 requires the usage of a counting modality, such 
as is used
in Counting MTL ($p$ denotes a heartbeat):
\begin{equation*}
	\always \left(start \rightarrow \left(\text{C}_{[120,180]}^{\geq 
		90}p\,\wedge\,\text{C}_{[120,180]}^{< 
		120}p\right)\right)
\end{equation*} 

On the other hand, to express that the heart rate increases by at
least 20\% when measured over consecutive and disjoint windows of 4
beats requires explicit clocks, such as used in XCTL, since the
beat-to-beat delay is variable ($x_i$'s are clocks):
\begin{align*}
	p\,\wedge (x_1=T)\,\wedge\, \eventually(
	p\,&\wedge ...\eventually
	(p\,\wedge\, (x_9=T)\,\wedge\\
	&\wedge\,(x_5-x_1)*0.8 \geq x_9-x_5 )) 
\end{align*}

As a final example, expressing that a threshold $a >0 $ for peak 
detection
is reset as a function of the previous peak value requires us to
remember the value of the peak.  
This necessitates memory registers,
or \emph{freeze quantification} of state variables, such as used in
Constraint LTL with Freeze Quantification $\CLTLF$ ($\freeze$ denotes
the freeze quantifier):
\begin{eqnarray*}
	\always (y > a \implies \freeze_{BL=1} \eventually  \left( 
	\formula_{\text{local-max}} \implies  a = 0.8z_2 \right))
	\\
	\formula_{\text{local-max}} \defeq  \freeze_{z_1=y} \nxt 
	(\freeze_{z_2=y} \nxt (z_2 > z_1 \land z_2> y))
\end{eqnarray*}	
This variety of logics required for these simple tasks, all of which
are fundamental building blocks of ICD operation, means that we
have already lost the unifying view of the entire problem. 

\paragraph{Heart rate}
The average heart rate, averaged over a moving window of size $L$, can be calculated by a QRE.

The QRE $peaks = Lip_{\alpha_0}$ returns a 1 if the the neighborhood it processed had a peak, and 0 otherwise.
If it is fed a string of length which is a multiple of $S \defeq (m+1)(N+1)$, e.g. $\Nc(0:\Delta)\Nc(\Delta:2\Delta)$, we need it to provide an answer only for the last neighborhood.
So we prepend it with a `do nothing' QRE $nothing$ which simply skips a string of length $S$, i.e. we are interested in the QRE $nothing^*peaks$.\footnote{The syntactically correct way of writing this would be as follows: first, $nothing$ is of type QRE$((d\in D)^S,\emptyset,\reals^{|\Xc|})$ where, recall, $\Xc$ is the parameter set of $peaks$.
To skip any prefix whose length is a multiple of $S$ we use $iter[e\rangle (nothing)$ where $e$ is an unused parameter required by the syntax.
Finally to skip such prefix but match the last substream with $peaks$ we simply concatenate:  $heart\!-\!rate = split(iter[e\rangle (nothing) [\Xc\rangle peaks))$. 
Note that $nothing$ is providing the initialization of the parameters in $\Xc$ to $peaks$, which is why we chose its cost domain to be $\reals^{|\Xc|}$.
Note also that $iter[e\rangle (nothing)$ is of type QRE($(D^S)^*, \emptyset, C$) and $peaks$ is of type QRE($D^S, \Xc,\booleans$) so they are unambiguously concatenatable and split is defined for them. 
Moreover, $heart\!-\!rate$ is of type QRE:$((D^S)^*D^S, \emptyset, \booleans)$ so it obeys the typing rules of streaming composition.}

Next If we stream $nothing^*peaks$ (via stream composition) to a sliding window aggregator $\iter{avg}_{[L]}$ , we get the sliding window average of events in the input stream 
\[heart\!-\!rate \defeq nothing^*peaks \gg \iter{avg}_{[L]}\]
(The sliding aggregator computes the average in a window of size $L$ 
\emph{data items}, but because of uniform sampling of the electrogram 
and the fact that all neighbourhoods have the same number of samples, 
a fixed number of data items means a fixed duration for the window.)
The sliding window aggregator ignores null input items $\epsilon$.

\paragraph{Heart rate stability}
The sliding window standard deviation can be similarly computed, and is called the `stability' discriminator as it indicates whether the heart rate is stable (small variance) or unstable (large variance).

\paragraph{Rate comparison}
Given $heart\!-\!rate_A$ and $heart\!-\!rate_V$ which compute the average atrial and ventricular rates respectively, we may compare the two using
\[q_{V>A} = gt(q_{HR,V}, q_{HR, A})\]
where the operation $gt: \reals^2 \rightarrow \booleans$ simply returns True if its first argument is greater than or equal to its second argument, and False otherwise.


==> camera - Copy - Copy (2)/chapters/experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}
%\todo[inline]{give the QRE for MDT too as a figure}
We show the results of running peak detectors $\qre{peakWPM}$ and $\qre{peakWPB}$ on real patient data, obtained from a dataset of intra-cardiac electrograms.
We also specified a peak detector available in a commercial ICD \cite{icdbook} as \ac{QRE} $\qre{peakMDT}$, and show the results for comparison purposes.
The implmentation uses an early version of the StreamQRE Java library~\cite{MRAIK17}.
Comparing the runtime and memory consumption of different algorithms (including algorithms programmed in QRE) in a consistent and reliable manner requires running a compiled version of the program on a particular hardware platform.
No such compiler is available at the moment, so we don't report such performance numbers.

The results in this section should not be interpreted as definitively establishing the superiority of one peak detector over another, as this is not this paper's objective.
Rather, the objective is to highlight the challenges involved in peak detection for cardiac signals, an essential signal-processing task in many medical devices.
In particular, by highlighting how different detectors perform on different signals, it establishes the need for a formal (and empirical) understanding of their operation on classes of arrhythmias.
This prompts the adoption of a formal description of peak detectors for further joint analysis with discrimination.
%A secondary objective is to show the \acp{QRE} in action.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[height=1.2in]{figures/A176WPBnWAVs80thr400}
		\label{fig:VT WPM WPB p400}
		\caption{$\bar{p}\,=\,400$}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[height=1.2in]{figures/A176WPBnWAVs80thr150}	
		\label{fig:VT WPM WPB p150}
		\caption{$\bar{p}\,=\,150$}
	\end{subfigure}
	\caption{\small $\qre{peakWPM}$-detected peaks (red circles) and $\qre{peakWPB}$-detected peaks (black circles) on a VT rhythm.}
	\label{fig:VT WPM WPB}
\end{figure*}

%\begin{figure}[t]
%		\centering
%		\includegraphics[width=\linewidth]{figures/A176WPBnWAVs80thr400}
%		\caption{Rectified EGM of a \ac{VT} showing 
%		$\qre{peakWPM}$-detected peaks as red 
%			circles and $\qre{peakWPM}$ as black circles 
%			($\bar{p}\,=\,400$)}
%		\label{fig:A176WPBnWAVs80thr400}
%	\end{figure}	
%	%-----------------------------------------------------------------
%	\begin{figure}[t]
%		\centering
%		\includegraphics[width=\linewidth]{figures/A176WPBnWAVs80thr150}
%		\caption{$\qre{peakWPM}$ (red) and $\qre{peakWPB}$ (black) on VT signal 
%		($\bar{p}\,=\,150$)}
%		\label{fig:A176WPBnWAVs80thr150}
%	\end{figure}
%	%-----------------------------------------------------------------

Fig.~\ref{fig:VT WPM WPB} presents one rectified EGM signal of a \acf{VT} recorded from a patient. 
Circles (indicating detected time of peak) show the result of 
running $\qre{peakWPM}$ (red circles) and $\qre{peakWPB}$ (black circles). 
These results were obtained for $\bar{s} = 80$, $BL = 150$, and different 
values of $\bar{p}$.
The first setting of $\bar{p}$ (Fig.~\ref{fig:VT WPM WPB}~(a)) for both \acp{QRE} was chosen to yield the best performance.
This is akin to the way cardiologists set the parameters of commercial \acp{ICD}: they observe the signal, then set the parameters.
We refer to this as the \textit{nominal setting}.
Ground-truth is obtained by having a cardiologist examine the signal and annotate the true peaks.

We first observe that the peaks detected by $\qre{peakWPM}$ match the ground-truth; i.e., the nominal performance of $\qre{peakWPM}$ yields perfect detection.
This is not the case with $\qre{peakWPB}$.
Next, one can notice that the time precision of detected peaks with $\qre{peakWPM}$ is
higher than with $\qre{peakWPB}$ due to maxima lines tracing down to the zero scale. 
Note also that the results of \qre{peakWPM} are stable for various parameters settings. 
Improper thresholds $\bar{p}$ or scales $\bar{s}$ degrade 
the results only slightly (compare locations of red circles on 
Fig.~\ref{fig:VT WPM WPB} (a) with 
Fig.~\ref{fig:VT WPM WPB} (b)). 
By contrast, $\qre{peakWPB}$ detects additional false peaks 
(compare black circles in Figs.~\ref{fig:VT WPM WPB} (a) and (b)). 
%Finally, note that peak times found with $\qre{peakWPB}$ precede the actual peak times (e.g., black circles in Fig.~\ref{fig:A176WPBnWAVs80thr150}).
%This can be explained by the fact that $\qre{peakWPB}$ declares a peak when the local maximum of coefficient values passes the threshold value for the first time. This point does not always correspond to an actual peak.  
%=====================================================================
%WPM RESULTS                                                          
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[height=1.2in]{figures/A173WAVnWDTs100thr300}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[height=1.2in]{figures/A181WDTsnominal}	
	\end{subfigure}
	\caption{\small WPM and $\qre{peakMDT}$ running on a VF rhythm (left) and $\qre{peakMDT}$ running on an NSR rhythm (right).}
	\label{fig:VF WPM MDT}
\end{figure*}

Fig.~\ref{fig:VF WPM MDT} (left)
shows WPM (red circles) running on a Ventricular Fibrillation (VF) rhythm, which is a potentially fatal disorganized rhythm.
Again, we note that WPM finds the peaks.

\input{chapters/mdtresults}

==> camera - Copy - Copy (2)/chapters/formalDefQREsApdx.tex <==
\section{Formal definition of QREs}
\label{formalDefQREs}

For the reviewers' convenience, this appendix gives the formal definition of \acp{QRE}.

For a set $D$ known as the data domain, a \emph{data stream} is a
finite word $w\,{\in}\,D^*$ and a \emph{data language} is a subset
$L\,{\subset}\,D^*$.  Let $\Phi_D$ be a collection of predicates over
$D$ which is closed under the boolean connectives and for which there
exists a finite quantity $time_{\Phi{\rm -}sat}$ such that the
satisfiability of any predicate $\phi\,{\in}\,\Phi_D$ is mechanically
decidable in time less than $time_{\Phi-sat}$.  \emph{Symbolic
  unambiguous regular expressions} (or \acp{RE} for short) are defined recursively as follows:
%
\begin{enumerate}
\item $\epsilon$ is a regular expression and defines the language
  $\val{\epsilon} \defeq \{\epsilon\}$.
\item For each predicate $\phi\,{\in}\,\Phi_D$, $\phi$ is a regular
  expression that identifies the language
  $\val{\phi} \defeq \{d\,{\in}\,D\:{\such}\:\phi(d)\,\text{ holds }\}$.
\item For each pair of regular expressions $r_1, r_2$, if $\val{r_1}$
  and $\val{r_2}$ are disjoint, then $r_1\,{+}\,r_2$ is an \ac{RE} and
  $\val{r_1\,{+}\,r_2}\:{=}\:\val{r_1}\,{\cup}\,\val{r_2}$.
\item For each pair of regular expressions $r_1, r_2$, if $\val{r_1}$
  and $\val{r_2}$ are unambiguously concatenable\footnote{Two
    languages $L_1,L_2\,{\subset}\,D^*$ are unambiguously concatenatable
    if any $w\,{\in}\,L_1L_2$ can be uniquely decomposed into $w=w_1w_2$
    s.t. $w_i\,{\in}\,L_i$.}, then $r_1\,r_2$ is a regular expression and
  $\val{r_1\,r_2} = \val{r_1}\,\val{r_2}$.
\item If $r$ is a regular expression with unambiguously iterable
  language $\val{r}$\footnote{A language $L$ is unambiguously iterable
    if it is non-empty and for any $w\,{\in}\,L^*$ there exists a
    unique decomposition $w = w_1w_2\,{\ldots}\,w_k$
    s.t.~$w_i\,{\in}\,L$ for all $i\,{\leq}\,k$.}, then $r^*$ is an
  \ac{RE} with language $\val{r^*}=\val{r}^*$.
\end{enumerate}

Predicates in $\Phi_D$ are only allowed to examine individual data
values. This restriction guarantees the decidability of questions like
"are two regular expressions disjoint?".  These \acp{RE} will be the
basic way in which patterns are detected in the EGM data.  For
example, given the stream of voltage values $y$,
$(y\,{\leq}\,1)^*(y\,{\geq}\,1)^{200}$ matches any sub-stream that is
below 1, then above 1 for at least 200 samples.

In addition to matching \acf{RE} in the input stream, we need to perform numerical
computations on the sub-streams that match.  A \ac{QRE} augments an
\ac{RE} with \emph{operations} on data types, \emph{parameters} that
are used to pass values between operations, and \emph{regular combinators} that build
more complex \acp{QRE} from simpler \acp{QRE}.  We introduce each 
in turn.
\begin{itemize}
\item Let $\Tc = \{T_1,T_2,\ldots\}$ be a \emph{set of data
  types}. Typical examples include the reals $\reals$, the
  non-negative integers $\Ne$, the booleans $\booleans = \{true,
  false\}$ and  the set $\Me$ of multisets of real numbers.
\item Let $\opset$ be a \emph{set of operations}
  $\{op_1,op_2,\,{\ldots}\}$ on various types, each operation being a
  function of the form
  $op:\,T_1\,{\times}\,{\ldots}\,{\times}\,T_k\:{\rightarrow}\:T$.
  For example, $\opset\:{=}\,\{{+},\,{*},\,{\rm avg},\,x\,{<}\,y\}$ is a set
  of operations on the types $\Tc\,{=}\,\{\reals,\Ne, \booleans\}$.
\item Let $X\,{=}\,(p_1,p_2,\ldots)$ be a \emph{list of parameters}, each
  $p_i$ being of some type $T_i\,{\in}\,\Tc$.
\item A \emph{cost term} $\tau$ is defined using
  $\tau \defeq {p}\:{|}\:{t}\,{\in}\,{T}\:{|}\:op(\tau_1,{\ldots},\tau_k)$
  where $op\,{\in}\,\opset$.  A cost term encodes a mapping
  $\val{\tau}{:}\:{T_1}\,{\times}\,{T_2}\,{\times}{\ldots}{\times}\,{T_k}\:{\rightarrow}\:{T}$
  from parameter valuations $\bar v$ to costs $\val{\tau}(\bar v)$.
\end{itemize}

We denote a valuation of the parameters in $X$ by $\bar v$.  The
valuation $\bar v[p/p_0]$ equals $\bar v$ except at $p\,{\in}\,X$,
where $v_p$ is replaced by $p_0$.

Intuitively, a \ac{QRE} maps a string $w$ to a cost term $f(w)$.  When
a parameter valuation $\bar v$ is given, this then further evaluates
to a cost value in $C$. Formally, for a data domain $D\,{\in}\,\Tc$,
cost domain $C\,{\in}\,\Tc$ and a parameter sequence
$X\,{=}\,(x_1,x_2,{\ldots},x_k)$, a \ac{QRE} $f$ identifies a function
$\val{f}{:}\,D^*\:{\rightarrow}\:({T_1}\,{\times}\,{T_2}\,{\times}\ldots{\times}\,{T_k}\:{\rightarrow}\:{C})\,{\cup}\,\{\bot\}$,
where $\bot$ is the undefined value.

The domain of the \ac{QRE} is the set of strings where it is defined.
Thus each \ac{QRE} is associated with a \acf{RE} $r$ whose language is
the domain of $f$:
$\val{r}\,{=}\,\{w\,{\in}\,D^*\,{\such}\,\val{f}(w)\,{\neq}\,{\bot}\}$.
Following \cite{Alur2016} we write $f$\,{:}\,QRE($r,X,C)$ to indicate
that $f$ is a QRE with RE $r$, parameters $X$ and cost domain $C$.  We
now give the construction rules of \acp{QRE}.  Due to lack of space,
we will only give those constructions that we use in this paper and
refer the reader to \cite{Alur2016} for the full set of constructions.
See Fig.\ref{fig:qre illustrations} for illustrations of the following
definitions.
%
\begin{exmp}
\label{ex:runningApdx}
To illustrate the definitions, we use a simple running example. Let
$\egm{:}\:{\reals_+}\,{\rightarrow}\,\reals$ be a discrete-time signal
(not necessarily uniformly sampled).  The data stream consists of
tuples ${d}\,{=}\,(t,\,{\egm(t)})$ sampled from $\egm$, thus the data
domain is $D\,{=}\,{\reals_+}\,{\times}\,{\reals}$.  Once a \ac{QRE}
is formally defined, from that point onwards, we will occasionally be
less strict about the syntax for the sake of added clarity.
\end{exmp}

\paragraph{\rm\bf 1. Basic functions.}
If $\formula\,{\in}\,\Phi_D$ is a predicate and
$\lambda{:}\,{D}\,{\rightarrow}\,{C}$ is a cost function, then the
semantics of
${\formula}\,{?}\,{\lambda}\,{:}\,\,$QRE($\formula,{\emptyset},{C}$)
is defined as follows:
\[
\val{{\varphi}\,{?}\,{\lambda}}(w,\bar v) = \left \lbrace \begin{matrix}
\lambda(w) &\;& \text{ if }|w|=1 \text{ and } \formula(w) = true,
\\ \bot &\;& \text{ otherwise }
\end{matrix} \right.
\]

\begin{exmp}
Let ${\lambda_1}\,{:}\,(t,\egm(t))\,{\mapsto}\,1$ be the constant 1
function, then the following QRE
$f_1\,{=}\,(d.{\egm}\,{<}\,{-M}\,|\,{d.\egm}\,{>}\,{M})\,{?}\,{\lambda_1}$
matches data items with voltages larger than $M$ in absolute value and
evaluates to 1.  In other words, $f_1$ marks the occurrence of a data
item with $|d.\egm|>M$.  On the other hand,
$f_a\,{=}\,{d}\,{\in}\,{D}\,{?}\,|d.\egm|^2$ maps any item $d$ to the
square of its voltage.
\end{exmp}

\paragraph{\rm\bf 2. Cost operations.}
Operations from $\opset$ can combine the values of individual
\acp{QRE}.  E.g. $sum(f,g)(w,\bar v)$ will produce the value
$\val{f}(w,\bar v)+\val{g}(w,\bar v)$ if both $f$ and $g$ are defined
on $w$ (and will produce $\bot$ otherwise).  Formally, consider an
operation $op\,{\in}\,\opset$ and $f_i\,{:}\,{\rm
  QRE}(r_i,X_i,T_i),~i=1{\ldots}k$.  If the domains are equal
$\val{r_1}\,{=}\,\val{r_2}\,{=}\,\ldots\,{=}\,\val{r_k}$ and the
parameter lists are pair-wise disjoint
$X_i\,{\cap}\,X_j\;{=}\;{\emptyset}$ then
$op(f_1,\ldots,f_k)\,{:}\,{\rm QRE}(r_1, \cup_iX_i, C)$ is defined as
follows:
\[
\val{op(f_1,\ldots,f_k)}(w,\bar v) = \left \lbrace \begin{matrix}
op(\val{f_1}(w,\bar v),\ldots,\val{f_k}(w,\bar v)) &\;& \text{ if }\val{f_i}(w) \neq \bot \forall i
\\
\bot &\;& \text{otherwise}
\end{matrix}\right.\]

\begin{exmp}
Let $\mu$ be a QRE that computes the average of a stream of length
$N$, that is, $\val{\mu}(w,\bar v)\,{=}\,\sum_i w_i.\egm/N$, and
$\sigma_2$ be a QRE that computes the average of the values squared,
that is, $\val{\sigma_2}(w,\bar v)\,{=}\,\sum_iw_i.\egm^2/N$.  Then
the the variance (difference of the two) is computed as $var = {\it
  diff}(\sigma_2, \mu)$.
\end{exmp}

\paragraph{\rm\bf 3. Substitution.}
Let
$f\,{:}\,{\rm QRE}(r_f,X_f,T_f)$ and $g\,{:}\,{\rm QRE}(r_g,X_g,T_g)$
be a pair of \acp{QRE} with equal domain $\val{r_f} = \val{r_g}$ and let the parameter $x \in X_f$ of type $T_g$ be the only shared parameter between $X_f$ and $X_g$.
Informally, the expression $f[x/g]$ substitutes the result of applying $g$ on $w$ for $x$, before evaluating $f$.
Formally, if both $\val{f}(w)$ and $\val{g}(w)$ are defined
$\val{f[x/g]}(w,\bar v) = \val{f}(w, \bar v[x/int_g])$ where $int_g = \val{g}(w,\bar v)$.
Otherwise it is undefined.

\paragraph{\rm\bf 4. Conditional choice.}
If we wish to also mark the occurrence of absolute voltage values
smaller than $M$, then we can use a conditional as follows:
\[
f_{01}\defeq (f_1 \; {\rm else} \; \underbrace{(d.\egm > -M \;\land \; d.\egm
  <M)\,{?}\,\lambda_0}_{f_0})
\]
where $\lambda_0$ is the constant 0 function.  This accepts a data
item and outputs 1 if $|d.\egm| > M$ (via $f_1$), else it outputs 0 (via $f_0$).
Formally, if $f$ and $g$ are \acp{QRE} with disjoint domains then
$f\;{\it else}\;{g}\,{:}\,{\rm QRE}(r_f\,{+}\,r_g, X_f\,{\cup}\,{X_g},
T_f\,{\cup}\,{T_g}$) and is given by
\[
\val{f\;{\it else}\;g}(w,\bar v) = \left \lbrace \begin{matrix}
int_f &\;& \text{ if }int_f \neq \bot, \text{ and } 
\\
\val{g}(w,\bar v) &\;& \text{ otherwise }
\end{matrix} \right.
\]
with $int_f = \val{f}(w,\bar v)$ is the semantics of QRE $f$.

\paragraph{\rm\bf 5. Concatenation.}
While a cost operation combines costs of \acp{QRE} that match the same
input stream, a concatenation combines costs of \acp{QRE} that match
disjoint \emph{substreams} of the input stream.  We now define a
restricted version of concatenation that we use in this paper.  A more
general concatenation combinator is defined in \cite{Alur2016}.  Let
$f\,{:}\,{\rm QRE}(r_f,X_f,T_f)$ and $g\,{:}\,{\rm QRE}(r_g,X_g,T_g)$
be a pair of \acp{QRE} with unambiguously concatenatable domains and
such that $X_f\,{\cap}\,X_g\;{=}\,{\emptyset}$. 
Let $op\,{\in}\,\opset$ be a binary operation.  Then
$\splitop{op}(f,g)$ is a QRE of the form ${\rm QRE}(r_fr_g,
X_f\,{\cup}\,X_g, T_g)$.  If an input stream $w$ can be uniquely split
into $w\,{=}\,w_f w_g$ such that both $\val{f}(w_f)$ and
$\val{g}(w_g)$ are defined then
$\val{\splitop{op}(f,g)}(w)\,{=}\,op(\val{f}(w_f), \val{g}(w_g))$.
Otherwise it is undefined.

\begin{exmp}
Consider the operation $gt$ defined by $gt(x,y)\,{=}\,x\,{>}\,y$ which
evaluates to $true$ if $x\,{>}\,y$.  Then
$split-gt(d\,{\in}\,D\,{?}\,d.\egm, d\,{\in}\,D\,{?}\,d.\egm)$ splits
a stream of length two and returns the value true if the first
element's voltage is greater than the second element's voltage.
\end{exmp}

\paragraph{\rm\bf 6. Iteration.}

The analog of the Kleene's star operator $(\_)^*$ on regular
expressions is iteration.  Consider $f\,{:}\,{\rm QRE}(r,X,T)$ with
unambiguously iterable domain and $p$ a parameter of type $T$.  Then
$f^*\,{=}\,iter[p\rangle(f)$ is a \ac{QRE} of the form
${\rm QRE}(r^*, \{p\}, T)$. It is defined on the input stream $w$ if
the latter can be uniquely divided into $w=w_1w_2{\ldots}w_k$ such
that $\val{f}(w_i)$ is defined for every $i$.  Intuitively, $f^*$ will
first evaluate $f$ on $w_1$: $int_1\,{=}\,\val{f}(w_1,\bar v)$.  This
intermediate value is passed to the next iteration which computes
$int_2\,{=}\,\val{f}(w_2,\bar v[x/int_1])$.  And so on up to $k$.  Thus
each iteration passes its output to the next iteration which can use it.

%The second intermediate value is passed along to the third
%evaluation as a parameter, and so on up to $k$.
%
%Intuitively, $f^*$ evaluates $f$ on each substream $w_i$.  When
%evaluating $\val{f}(w_i)$, it uses the output of the previous
%evaluation (namely, $\val{f}(w_{i-1})$ to initialize the value of
%parameter $p$ in the current evaluation .  Thus $p$ serves to set the
%context for from one iteration to the next.

See Fig. \ref{fig:qre illustrations} for a graphical illustration
of iteration.  Formally, given a valuation
$\bar v$, the intermediate values $int_i$ are defined as follows:

\begin{itemize}
\item {\it Initialization:} $int_0 = v_p$, the value of $p$ under the valuation $\bar v$.
\item {\it Iteration:} $int_i = \val{f}(w, \bar v[p/int_{i-1}])$.
\item {\it Termination:} $\val{iter[x\rangle(f)}(w,\bar v) = int_k$.
\end{itemize}

It can be shown that this iterator can implement \acp{QRE} of type
$\iterop(f)$, where at each iteration, the value $op(int_{i-1},
\val{f}(w_i))$ is computed.  For example, sum, average, max, min,
etc.,~of a stream of numbers, is easily implemented.

\begin{exmp}
Say we want to count the number of data items whose absolute voltage
exceeds threshold $M$.  Then we are interested in $\iter{sum}(f_0)$,
which accepts a stream of values below the threshold and outputs 0
(recall that every match of $f_0$ produces a 0, thus their sum is 0).
We also need to iterate $\iter{sum}(f_1)$, which will match
$(|d.\egm|\,{>}\,{M})^*$ and output the length of the matching stream.
We then concatenate the two: $\iter{sum}(f_0)\cdot \iter{sum}(f_1)$
will match $(|d.\egm|\,{\leq}\,M)^*(|d.\egm|\,{>}\,M)^*$ and output
the number of times the threshold was exceeded.  Finally, we iterate
that last QRE over the entire stream.
\end{exmp}

\paragraph{\rm\bf 7. Stream composition.}
Very often we are interested in generating intermediate streams $z \in
C^*$ from the data stream $w \in D^*$.  These can then be further
processed by other \acp{QRE} to produce a final cost term. In our
running exmaple, $f_{01}$ can produce a stream of 0s and 1s which is
further processed.  Streaming composition achieves this.  Let
$f\,{:}\,{\rm QRE}(r_f,\emptyset,T_f)$ and $g\,{:}\,{\rm
  QRE}(T_f^*,X_g,T_g)$ be a pair of \acp{QRE}.  Note that $g$ is
defined over all intermediate data streams produced by $f$.  Then
$f\,{\gg}\,{g}\,{:}\,{\rm QRE}(D^*,X_g,T_g)$.  Given the input stream
$w=w_1w_2{\ldots}w_k$ and parameter valuation $\bar v$, define the
intermediate results $int_i$, $i\,{\leq}\,k$, as follows:

\begin{itemize}
\item {\it If}\;\;$\val{f}(w_1w_2{\ldots}w_i, \bar v)\,{\neq}\,\bot$ then
  $int_i\,{=}\,\val{f}(w_1w_2{\ldots}w_i, \bar v_{\emptyset})$ where
  $\bar v_{\emptyset}$ is the empty parameter valuations.
\item {\it Otherwise} $int_i =\epsilon$.
\item {\it Finally} $\val{f \gg g}(w,\bar v) = \val{g}(int_1 int_2 \ldots int_k, \bar v)$.
\end{itemize} 


%QREs do place some restrictions on the basic predicates and how costs are 
%combined. 
%Most notably, 
%These will be reviewed later, and are motivated by the desire to 
%maintain decidability of fundamental questions like: are two REs 
%equivalent? and to obtain reasonable complexity for computing the 
%value of a QRE.
%Because our concerns in this paper are mainly about the performance 
%of runtime monitoring, we will feel free to relax some of the 
%restrictions that are mainly motivated by decidability questions, 
%without straying far from the QRE philosophy.


==> camera - Copy - Copy (2)/chapters/fourierBlurb.tex <==
\begin{figure}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{figures/sin_fft}
	\caption{Signal of Fig.~\ref{fig:sin_signal} in Fourier domain}
	\label{fig:sin_fft}
\end{figure}
To analyze the properties of a stationary signal $\egm: \reals_+ \rightarrow \reals$, it is convenient to decompose it into its harmonics, which are sinusoids with a particular phase and frequency. 
Since $e^{iwt} = \cos wt + i\sin wt$, the signal can equivalently be decomposed into a sum of complex exponentials.
This is accomplished through the use of the \emph{Fourier Transform}~\cite{waveletMallat}: 
%% ($i=\sqrt{-1}$)
\begin{equation}
\label{eq:fourier pair}
\hat{\egm}(w)=\int\limits_{-\infty}^{+\infty}\egm(t)e^{-iwt}\,dt,
\qquad
\egm(t)=\frac{1}{2\pi}\int\limits_{-\infty}^{+\infty}\hat{\egm}(w)
e^{iwt}\,dw
\end{equation}
$\hat{\egm}(w)$ is called the Fourier transform of $\egm(t)$.
Eq.~\eqref{eq:fourier pair} proves that the transform is invertible and so the signal is uniquely determined by either its time-domain or Fourier-domain description.
Parameter $w$ is the frequency: $|\hat{\egm}(w)|$ gives the power of the signal at frequency $w$. 
Thus, the larger $|\hat{\egm}(w)|$, the more energy is contained at that frequency. 

For example, the signal $\egm(t)$ in Fig.~\ref{fig:sin_signal} 
contains three distinct regimes of variation at different 
frequencies.
The first regime contains two periods of a slow (5Hz frequency) sinusoid, the second contains fifteen periods of fast (10 Hz) sinusoid, and the third contains the superposition (linear composition) of the first with a very fast (35 Hz) sinusoid. 
The fast harmonics in the last regime can be thought of as constituting noise. 
The Fourier transform of $\egm(t)$ is depicted in
Fig.~\ref{fig:sin_fft} and shows three large components at the 
frequencies 5, 10 and 35 Hz.
The frequency domain provides a very intuitive way of capturing the harmonics of a signal, and the Fourier Transform is a tool for bringing these harmonics to light. 
In contrast, writing a temporal formula capturing a signal of one or several frequencies is impractical.

The Fourier transform gives the frequency content, but \emph{does not localize it in time}. 
Looking at Fig.~\ref{fig:sin_fft}, one cannot further specify whether the 35 Hz component occurs early or late in the signal.
A solution would be to take a Fourier transform in a sliding window of the signal, but this raises questions of which windowing function to use, how wide it should be, the amount of overlap between windows, etc.

==> camera - Copy - Copy (2)/chapters/future.tex <==
\section{Conclusions and Future Work}
\label{sec:future}

The tasks of discrimination and peak detection, fundamental to arrhythmia-discrimination algorithms, are easily and succinctly expressible in \acp{QRE}. 
One obvious limitation of \acp{QRE} is that they only allow regular matching, though this is somewhat mitigated by the ability to chain QREs (though the streaming combinator $\gg$) to achieve more complex tasks.
%This was demonstrated with three peak-detection algorithms and with several discriminators.  
One advantage of programming in \acp{QRE} is that it automatically provides us with a base implementation, whose time and memory complexity is independent of the stream length.

As future work, it will be interesting to compile a QRE into C or assembly code to measure and compare actual performance on a given hardware platform.
Also, just like an RE has an equivalent machine model (DFA), 
a \ac{QRE} has an equivalent machine 
model in terms of a deterministic finite-state transducer~\cite{Alur2016}.
This points to an analysis of a 
QRE's correctness and efficiency beyond testing.
Two lines of inquiry along these lines are promising in the 
context of medical devices.

\textbf{Probabilistic analysis.}
Assume a probabilistic model of the \ac{QRE}'s input strings.
%input strings $w$ are drawn from some probability distribution supported on $D^*$. 
For medical devices, such a model might be learned from data.
We may then perform a statistical analysis of the output of the \ac{QRE} under such an input model. 
% to estimate the average number of computations required to obtain an answer, the probability of computing a given value, etc.
%Such statistics have direct relevance to the study of medical devices.
In particular, we may estimate how long it takes the ICD to detect a fatal arrhythmia, or the probability of an incorrect detection by the ICD.

\textbf{Energy calculations.}
We may compute the energy consumption of an algorithm that is expressed as a QRE, by viewing consumption as another quantity computed by the QRE.
Alternatively, we may label the transitions of the underlying DFA by ``energy terms", and levarage analysis techniques of weighted automata to analyze the energy consumption.
Energy considerations are crucial to implanted medical devices that must rely on a battery, and which require surgery to replace a depleted battery.
%given a stochastic model of its input, we may study the statistical performance of a ac{QRE} on that inpput model.
%Models of the physiological input signals, such as cardiac electrograms, must be able to reproduce the variability displayed by a given patient accross time, and the variability between patients.
%Thus, and given the absence of workable mechanistic models to explain this variability, the models need to be learned from data.
%This typically implies learning of a stochastic model, since the great variability in the signals can be approximated using probabilistic evolution.
%For example, we can show that if the input data is i.i.d, and the SSTT does not use parameters, then the output of the SSTT is a Discrete Time Markov Chain, on which we may perform probabilistic model checking.

%\textbf{Distance between QREs.}
%Here one needs an appropriate notion of distance between two signals (e.g., EGMs or the output of $\qre{peakWPM}$, $\qre{peakWPB}$ or $\qre{peakMDT}$), and gradually generalize this to a  distance between two QRES.
%For example, a generalized Skorokhod distance was used in \cite{AbbasF14_Conformance} to quantify the value and time mismatches between trajectories of hybrid systems.
%In~\cite{MajumdarP15}, a Skorokhod distance was used to quantify these mismatches between continuous signals by allowing the application 
%of time distortions to minimize their pointwise distance.  
%The work in~\cite{MajumdarP16} extends the definition of this distance to sets of signals in the form of \emph{flow-pipes}. 
%Recent work in~\cite{Jaksic2016} defines a proper distance between two discrete-time, discrete-domain signals, and between a signal of this type and a Signal Temporal Logic (STL) specification. 
%Given a set of EGMs whose peaks have been annotated by a team of cardiologists (this set of ground-truth is always going to be finite), we can readily compare the \textit{outputs} of two \acp{QRE} processing these same inputs (for example, \qre{peakWPM} vs \qre{peakWPB} vs \qre{peaMDT}) using the notion of distance in~\cite{Jaksic2016}. 
%Generalizing this comparison to two \acp{QRE} will be more challenging, and it should both generalize the finitary case and take advantage of the structure of the QREs. 

%We have demonstrated that peak detection, a common and essential signal processing task, cannot be specified in temporal (or time-frequency) logic.
%We leveraged a characterization of peaks as singularities in the wavelet domain, formalized it using \acfp{QRE}, and demonstrated its performance on real patient electrograms.
%In other work, we use this peak characterization in order to specify various arrhythmia discriminators of ICDs in QREs. 
%Finally, it would be very interesting to consider what kind of compile- or run-time analysis questions (e.g., refinement, prediction, and control) can be answered for \acp{QRE} in the specific context of \ac{ICD} verification.


==> camera - Copy - Copy (2)/chapters/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Medical devices blend signal 
processing (SP) algorithms with decision algorithms such that the performance and correctness of the latter critically depends on that of the former.  
As such, analyzing a device's decision making in isolation of SP offers at best an incomplete picture of the device's overall behavior.  
For example, an \ac{ICD} will 
first perform \textit{Peak Detection} (PD) on its input voltage signal, also known 
as an \textit{electrogram} (see Fig.~\ref{fig:nsr and its cwt}). 
The output of PD is a timed boolean signal where a~1 indicates a peak (local extremum) produced by a heartbeat,
%, i.e., a local maximum or minimum,
which is used by the downstream \textit{discrimination algorithms} to differentiate between fatal and 
non-fatal rhythms.
%Each such discriminator computes a feature of the timed boolean signal, such as median heart rate, to make a Fatal vs. Non-Fatal decision.
%The overall decision  is composed of all the discriminators' decisions.
%For example, the \textit{V-rate} discriminator computes the median of the heart rate in a sliding window fashion and compares it to a threshold to make its decision.
%Potentially fatal rhythms receive device therapy to terminate them, while the non-fatal rhythms are left to terminate on their own.
%The accuracy of PD directly affects the correctness of the overall arrhythmia detector.
Over-sensing (too many false peaks detected) and under-sensing (too many true peaks missed) can be responsible for as much as 10\% of an ICD's erroneous decisions~\cite{Swerdlow14_SensingTroubleshooting}, as they lead to inaccuracies in estimating the heart rate and in calculating important timing relations between the beats of the heart's chambers.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[height=1.2in]{figures/A173NSR}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[height=1.2in]{figures/A173NSRSpgrm}	
	\end{subfigure}
	\caption{\small Rectified EGM during normal rhythm (left) and its CWT spectrogram (right)}
	\label{fig:nsr and its cwt}
\end{figure*}

Motivated by the desire to verify ICD algorithms for cardiac 
arrhythmia discrimination, \textit{we seek a unified formalism for expressing and analysing the PD and discrimination tasks commonly found in ICD algorithms.}
%Note that PD is a fundamental SP primitive in its own right. 
A common approach would be to view these tasks as one of checking that the cardiac signal satisfies certain requirements, express these requirements in temporal logic, and obtain the algorithms by monitor synthesis. 
For example, PD evaluates to~1 if the signal (in an observation window) contains a peak, 
while the \textit{V-Rate} discriminator evaluates to~1 if the average heart rate exceeds a certain threshold. 

As discussed in Section~\ref{sec:manylogics}, however, this approach quickly leads to a fracturing of the formalisms: PD algorithms and the various discriminators require different logics, and some simply cannot be expressed succinctly (if at all) in any logic available today.
%The need for different logics implies the loss of a unifying formalism for analysis, since their relative expressive powers are not all known.
Thus, despite the increasingly sophisticated variety of temporal logics that have appeared in the literature~\cite{Donze2012,BrimDSV14}, they are inadequate for expressing the operations of PD and discrimination succinctly.
It should be noted that PD is an extremely common signal-processing primitive used in many domains, and forms of discrimination appear in several cardiac devices besides ICDs, such as Implantable Loop Recorders and pacemakers.
Thus the observed limitations of temporal logics extend beyond just ICD algorithms.

PD and discrimination both require reasoning, and performing a wide range of numerical operations, over data streams, where the data stream is the incoming cardiac electrogram observed in real-time.
For example, a commercial peak detector (demonstrated in Section~\ref{sec:experiments}) defines a peak as a value that exceeds a certain time-varying threshold, and the threshold is periodically re-initialized as a percentage of the previous peak's value.
As another example, the \textit{Onset} discriminator compares the average heart rate in two successive windows of fixed size.
Thus, the desired formalism must enable value storage, time freezing, various arithmetic operations, and nested computations, \textit{while remaining legible and succinct, and enabling compilation into efficient implementations}.

We therefore propose the use of \acfp{QRE} to describe 
(three different) peak detectors and a common subset of discriminators.
\acp{QRE}, described in Section~\ref{sec:qre primer}, are a \textit{declarative} formal language based on classical regular expressions for specifying \textit{complex numerical 
queries on data streams}~\cite{Alur2016}.
\acp{QRE}' ability to interleave user-defined computation at any 
nesting level of the underlying regular expression gives them significant expressiveness.
(Formally, \acp{QRE} are equivalent to the streaming composition of regular functions~\cite{AlurFR2014}).
\acp{QRE} can also be compiled into runtime- and memory-efficient implementations, which is an important consideration for implanted medical devices.

To demonstrate the versatility and suitability of \acp{QRE} for our task, we focus on PD in the rest of the paper, since it is a more involved than any single discriminator.
Three different peak detectors are considered (Section~\ref{sec:peaks in wav domain}): 
\begin{inparaenum}
	\item detector WPM, which operates in the wavelet domain,% and which we have slightly adapted to the discrete-time setting, 
	\item detector WPB, our own modification of WPM that sacrifices accuracy for runtime, and
	\item detector MDT, which operates in the time domain, and is implemented in an \ac{ICD} on the market today. 
\end{inparaenum}
For all three, a \ac{QRE} description is derived (Section~\ref{sec:qre PD}).
The detectors' operations is illustrated by running them on real patient electrograms (Section~\ref{sec:experiments}).

In summary, our contributions are:
\begin{itemize}
	\item We show that a common set of discriminators is easily encoded as \acp{QRE}, and compare the \acp{QRE} to their encoding in various temporal logics.
	\item We present two peak detectors based on a general wavelet-based characterization of peaks.
	\item We show that the wavelet-based peak detectors, along with a commercial time-domain peak detector found in current ICDs, are easily
%, succinctly 
and clearly expressible in \acp{QRE}. 
	\item We implement the \acp{QRE} for peak detection and demonstrate their capabilities on real patient data.
\end{itemize}


%The rest of the paper is organized as follows.  
%Section~\ref{sec:manylogics} compares the use of \acp{QRE} and temporal logics in expressing discrimination and peak detection operations, and serves as a soft introduction to \ac{QRE} and establishing their ease of use and suitability for the task. 
%Section~\ref{sec:peaks in wav domain} presents \textit{WPM} and \textit{WPB}, the wavelet-based characterizations of peaks.  
%Section~\ref{sec:qre primer} offers a primer on QREs, while Section~\ref{sec:PD} presents \textit{peakWPM} and \textit{peakWPB}, our QRE-based formalizations of \textit{WPM} and \textit{WPB}, respectively.  
%Section~\ref{sec:experiments} compares the performance of the \textit{peakWPM}, \textit{peakWPB} and \textit{peakMDT} PD algorithms on real patient data.  
%Section~\ref{sec:relatedWork} discusses related work, 
%and Section~\ref{sec:future} offers concluding remarks and a number of directions for future work.


%A joint analysis of the two types of tasks (SP and disciminators) is challenged by the fact that they are 
%typically expressed in different mathematical languages.
%Speaking somewhat simplistically, SP tasks like PD are described and 
%analyzed in the language of applied analysis. 
%The correctness of decision procedures over boolean signals is 
%usually approached using temporal logics and automata, with reference 
%to some specification of correctness.
%The language of SP is usually not amenable to formal analysis of the 
%sort appropriate for determining formal correctness of the overall 
%ICD algorithm (PD and discriminators together).
%In fact, in most SP applications, the ultimate criterion for whether 
%the algorithm performed well remains the subjective judgement of a 
%domain expert.
%This is true of peak detectors used in ICDs as well: ultimately, a 
%cardiologist determines whether the detected peaks are indeed 
%indicative of a heartbeat or not. 
%However, given a generative model of the electrogram (which is the 
%input signal to the ICD), it does make sense to pursue a formal 
%correctness and performance analysis of the \textit{overall} 
%algorithm, for which a correctness specification \textit{can} be 
%developed.



==> camera - Copy - Copy (2)/chapters/mdtresults.tex <==
%\subsection{Results of commercial \large{$\qre{peakMDT}$}}
%\label{sec:mdtresults}
Detector MDT works almost perfectly with nominal parameters settings on 
any Normal Sinus Rhythm (NSR) signal (see Fig.~\ref{fig:VF WPM MDT} right). 
NSR is the ``normal" heart rhythm.
The detected peak times are slightly early because $\qre{peakMDT}$ declares a peak when the signal exceeds a time-varying threshold, rather than when it reaches its maximum.
Using the same 
nominal parameters on more disorganized EGM signals with higher 
variability in amplitude, such as VF, does not produce proper 
results; see the black circles in Fig.~\ref{fig:VF WPM MDT} left.
%Other possible values of 
%parameters (blanking period and minimal threshold) improve $\qre{peakMDT}$ results, but still produce false positives; see 
%Fig.~\ref{fig:A173MDTBL250minThr80} (additional peaks are detected 
%around $1500$ms and $2250$ms). 


==> camera - Copy - Copy (2)/chapters/qrePD.tex <==
%\input{formalDefQREs}
\section{QRE Implementation of Peak Detectors}
\label{sec:qre PD}
We now describe the QREs that implement peak detectors WPM and WPB of Section~\ref{sec:waveletsForPD}.
It is emphasized that even complicated procedures such as these two algorithms can be described in a declarative fashion using \acp{QRE}, without resorting to a programming language or explicitly storing state, etc.

\input{chapters/qrepeakWPM}
\input{chapters/qrepeakWPB}
 






==> camera - Copy - Copy (2)/chapters/qrePrimer.tex <==
\section{A QRE Primer}
\label{sec:qre primer}

\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.3]{figures/QREs2_new.pdf}
	\caption{{\small QREs and their combinators. 
			a)~Basic QRE $\varphi?\lambda$ matches one data item $d$ and evaluates to $\lambda(d)$ if $\varphi(d)$ is True. b)~QRE $op(f_1,\ldots,f_k)$ evaluates the $k$ QREs $f_1,\ldots,f_k$ on the same stream $w$ and combines their outputs using operation $op$ (e.g., addition). $f_i$ outputs a value of type $T_i$. 
		c)~QRE $f\; else\; g$ evaluates to $f$ if $f$ matches the input stream; else it evaluates to $g$. 
		d)~QRE $\splitop{op}(f,g)$ splits its input stream in two and evaluates $f$ on the prefix and $g$ on the suffix; the two results are then combined using operation $op$. 
		e)~QRE $iter[p\rangle\!(f)$ iteratively applies $f$ on substreams that match it, analogously to the Kleene-$^*$ operation for REs. Results are passed between iterations using parameter $p$.
		f)~QRE $f \gg g$ feeds the output of QRE $f$ into QRE $g$ as $f$ is being computed. }}
	\label{fig:qre illustrations}
\end{figure*}

An examination of discrimination and PD (Sections~\ref{sec:manylogics} and~\ref{sec:peaks in wav domain}) shows the need for a language that:
1)~Allows a rich set of numerical operations.
2)~Allows  matching of complex patterns in the signal, to select scales and frequencies at which interesting structures exist. 
3)~Supports the synthesis of time- and memory-efficient implementations.
%Since regular expressions (RE) are equivalent to Linear Temporal Logic formulas (LTL) when expressing bounded-time temporal properties, and at least as widely used as LTL, 
This led to the consideration of \acfp{QRE}. 
A \ac{QRE} is a symbolic regular expression over a data domain $D$, augmented with data
costs from some cost domain $C$.  
A \ac{QRE} views the signal as a
\emph{stream} $w\in D^*$ that comes in one data item at a time. As the Regular Expression (RE) matches
the input stream, the cost of the \ac{QRE} is evaluated.

% \begin{exmp}
% 	\label{ex:first}
% 	Assume that a discrete-time voltage signal comes in as stream of values $(y_i)_{i\in \Ne}$.
% 	We want to count the
% 	number of samples that exceed a certain threshold
% 	${\theta}\,{\in}\,{\reals}$. 
% 	To do this, we need to first use QRE 
% 	%
% 	$\qre{count}\!\defeq\!(y\,{>}\,{\theta}\,{?}\,1)\;else\;(y \leq \theta?0)$
% 	%
% 	to produce a~1 whenever the current sample exceeds the threshold,
% 	and~0 otherwise.  This matches the \emph{symbolic} Regular Expression (RE)
% 	%
% 	$(y\,{>}\,{\theta}\,|\,y\,{\leq}\,{\theta})$,
% 	%
% 	where the word "symbolic" highlights the fact that the
% 	basic match is a predicate on the data item $y$ (here, the predicates are $y>\theta$ and $y \leq \theta$).  
% 	Second, to count how
% 	many samples exceed the threshold, we would like to sum the output stream of
% 	this expression; so, we use the \emph{quantitative} regular expression
% 	%
% 	$\qre{aboveTh} \defeq\iter{sum}(\qre{count})$,
% 	%
% 	which \emph{iterates} the $\qre{count}$ QRE and \emph{adds} each
% 	new result to the accumulating sum.  In this case, the data domain
% 	$D=\reals$ and the cost domain $C = \Ne$.  The \emph{sum} operation
% 	combines the costs of subexpressions.
% \end{exmp}

%A \ac{QRE} augments an
%\ac{RE} with \emph{operations} on data types, \emph{parameters} that
%are used to pass values between operations, and \emph{regular combinators} that build
%more complex \acp{QRE} from simpler \acp{QRE}. 
Formally, consider a set of types $\Tc = \{T_1,T_2,\ldots ,T_k\}$, a data domain $D\,{\in}\,\Tc$,
a cost domain $C\,{\in}\,\Tc$, 
and a parameter set
$X\,{=}\,(x_1,x_2,{\ldots},x_k)$, where each $x_i$ is of type $T_i$.
Then a \ac{QRE} $f$ is a function
\[\val{f}{:}\,D^*\:{\rightarrow}\:({T_1}\,{\times}\,{T_2}\,{\times}\ldots{\times}\,{T_k}\:{\rightarrow}\:{C})\,{\cup}\,\{\bot\}\]
where $\bot$ is the undefined value.
Intuitively, if the input string $w \in D^*$ does not match the RE of $f$, then $\val{f}(w) = \bot$.
Else, $\val{f}(w)$ is a function from ${T_1}\,{\times}\,{T_2}\,{\times}\ldots{\times}\,{T_k}$ to $C$. 
%Note that whether $f$ is defined depends only on the input stream $w \in D^*$, and not on the parameter valuation.
%Intuitively, a \ac{QRE} maps a string $w\in D^*$ to a cost function $\val{f}(w)$.
When
a parameter valuation $\bar v \in {T_1}\,{\times}\ldots{\times}\,{T_k}$ is given, this then further evaluates
to a cost value in $C$, namely $\val{f}(w)(\bar v)$. 
Fig.~\ref{fig:qre illustrations} provides an overview of \acp{QRE} and their combinators.

%% COMPILATION
\acp{QRE} can be compiled into efficient \textit{evaluators} that process each
data item in time (or memory) polynomial in the size of the \ac{QRE}
and proportional to the maximum time (or memory) needed to perform an \emph{operation} on a set of cost terms, such as addition, least-squares, etc.
The operations are selected from a set of operations \emph{defined by the user}.
\textit{It is important to be aware that the choice of operations constitutes a trade-off between expressiveness (what can be computed) and complexity (more complicated operations cost more).}
%Memory and computation time are very important considerations for ICDs, which must react to fatal rhythms very quickly while having a very limited on-chip memory.
See~\cite{Alur2016} for restrictions placed on the predicates and the symbolic regular expressions.

The declarative nature of \acp{QRE} will be important when writing complex algorithms, without having to explicitly maintain state and low-level data flows.
But as with any new language, \acp{QRE} require some care in their usage. 
Space limitations preclude us from giving the formal definition of \acp{QRE}.
Instead, we will describe what each \ac{QRE} does in the context of peak detection to give the reader a good idea of their ease of use and capabilities.
Fig.~\ref{fig:qre illustrations} illustrates how 
\acp{QRE} are defined and what they compute.
%For the reviewers' convenience, we have included the formal 
%definition along with more examples in an appendix at the end of this 
%paper. Reviewers who wish so can consult it for more background. In 
%the final version of the paper this appendix will be moved online.
Readers familiar with \acp{QRE} will notice that, when writing the QRE expressions, we occasionally sacrifice strict syntactic correctness for the sake of presentation clarity.

%% S R E
%The regular expressions used in \acp{QRE} are  \emph{symbolic
%	unambiguous regular expressions} (or \acp{RE} for short).
%These are defined recursively in the same way as traditional regular expressions, with two differences: first, the base case uses predicates $\formula$ over $D$ from some set of predicates $\Phi_D$ (whence the name `symbolic'):
%%
%\begin{enumerate}
%	\item (Base case 1) $\epsilon$ is a regular expression and defines the language
%	$\val{\epsilon} \defeq \{\epsilon\}$.
%	\item (Base case 2) For each predicate $\phi\,{\in}\,\Phi_D$, $\phi$ is a regular
%	expression that identifies the language
%	$\val{\phi} \defeq \{d\,{\in}\,D\:{\such}\:\phi(d)\,\text{ holds }\}$.
%\end{enumerate}
%%
%And secondly, only REs with unambiguously concatenatable languages\footnote{Two
%	languages $L_1,L_2\,{\subset}\,D^*$ are unambiguously concatenatable
%	if any $w\,{\in}\,L_1L_2$ can be uniquely decomposed into $w=w_1w_2$
%	s.t. $w_i\,{\in}\,L_i$.} are allowed in a concatenation $r_1 r_2$,  
%and only an RE with unambiguously iterable language\footnote{A language $L \subset D^*$ is unambiguously iterable
%	if it is non-empty and for any $w\,{\in}\,L^*$ there exists a
%	unique decomposition $w = w_1w_2\,{\ldots}\,w_k$
%	s.t.~$w_i\,{\in}\,L$ for all $i\,{\leq}\,k$.} is allowed in a Kleene-$^*$ operation $r^*$.
%
%Predicates in $\Phi_D$ are only allowed to examine individual data
%values. This restriction guarantees the decidability of questions like
%"are two regular expressions disjoint?".  
%These \acp{RE} will be the basic way in which patterns are detected in the signal.  

%% OPS
%In general, one can use any of a pre-defined set of operations to combine the costs of sub-QREs.
%The ability to specify a set of operations (like min, max, average, 
%etc.) and to interleave these operations at any nesting level gives
%\acp{QRE} great expressive power.  
%QREs allow the use of a \emph{declarative} style which makes
%it easier to maintain a global view of the stream and of the required
%calculations.

%For a set $D$ known as the data domain, a \emph{data stream} is a
%finite word $w\,{\in}\,D^*$ and a \emph{data language} is a subset
%$L\,{\subset}\,D^*$.  Let $\Phi_D$ be a collection of predicates over
%$D$ which is closed under the boolean connectives and for which there
%exists a finite quantity $time_{\Phi{\rm -}sat}$ such that the
%satisfiability of any predicate $\phi\,{\in}\,\Phi_D$ is mechanically
%decidable in time less than $time_{\Phi-sat}$. 

%In addition to matching \acf{RE} in the input stream, we need to perform numerical
%computations on the sub-streams that match.  A \ac{QRE} augments an
%\ac{RE} with \emph{operations} on data types, \emph{parameters} that
%are used to pass values between operations, and \emph{regular combinators} that build
%more complex \acp{QRE} from simpler \acp{QRE}.  We introduce each 
%in turn.
%\begin{itemize}
%	\item Let $\Tc = \{T_1,T_2,\ldots\}$ be a \emph{set of data
%		types}. Typical examples include the reals $\reals$, the
%	non-negative integers $\Ne$, the booleans $\booleans = \{true,
%	false\}$ and  the set $\Me$ of multisets of real numbers.
%	\item Let $\opset$ be a \emph{set of operations}
%	$\{op_1,op_2,\,{\ldots}\}$ on various types, each operation being a
%	function of the form
%	$op:\,T_1\,{\times}\,{\ldots}\,{\times}\,T_k\:{\rightarrow}\:T$.
%	For example, $\opset\:{=}\,\{{+},\,{*},\,{\rm avg},\,x\,{<}\,y\}$ is a set
%	of operations on the types $\Tc\,{=}\,\{\reals,\Ne, \booleans\}$.
%	\item Let $X\,{=}\,(p_1,p_2,\ldots)$ be a \emph{list of parameters}, each
%	$p_i$ being of some type $T_i\,{\in}\,\Tc$.
%	\item A \emph{cost term} $\tau$ is defined using
%	$\tau \defeq {p}\:{|}\:{t}\,{\in}\,{T}\:{|}\:op(\tau_1,{\ldots},\tau_k)$
%	where $op\,{\in}\,\opset$.  A cost term encodes a mapping
%	$\val{\tau}{:}\:{T_1}\,{\times}\,{T_2}\,{\times}{\ldots}{\times}\,{T_k}\:{\rightarrow}\:{T}$
%	from parameter valuations $\bar v$ to costs $\val{\tau}(\bar v)$.
%\end{itemize}
%
%Intuitively, a \ac{QRE} maps a string $w$ to a cost term $\val{f}(w)$.  When
%a parameter valuation $\bar v$ is given, this then further evaluates
%to a cost value in $C$, namely $\val{f}(w,\bar v)$. 
%Formally, for a data domain $D\,{\in}\,\Tc$,
%cost domain $C\,{\in}\,\Tc$ and a parameter sequence
%$X\,{=}\,(x_1,x_2,{\ldots},x_k)$, a \ac{QRE} $f$ identifies a function
%$\val{f}{:}\,D^*\:{\rightarrow}\:({T_1}\,{\times}\,{T_2}\,{\times}\ldots{\times}\,{T_k}\:{\rightarrow}\:{C})\,{\cup}\,\{\bot\}$,
%where $\bot$ is the undefined value.
%Note that whether $f$ is defined depends only on the input stream $w \in D^*$.
%
%The domain of the \ac{QRE} is the set of strings where it is defined.
%Thus each \ac{QRE} is associated with a \acf{RE} $r$ whose language $\val{r}$ is
%the domain of $f$:
%$\val{r}\,{=}\,\{w\,{\in}\,D^*\,{\such}\,\val{f}(w)\,{\neq}\,{\bot}\}$.



==> camera - Copy - Copy (2)/chapters/qrepeakWPB.tex <==
%=====================================================================
\subsection{QRE Implementation of WPB}
\label{sec:qre wpb}
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.25]{figures/WPB}
	\caption{QRE $\qre{peakWPB}$}
	\label{fig:WPB}
\end{figure}

Peak characterization WPB of 
Section~\ref{sec:waveletsForPD} is implemented as \ac{QRE} $\qre{peakWPB}$.
See Fig.~\ref{fig:WPB}.
The input data stream is the same as before.
\begin{itemize}
	\item QRE $\qre{oneMax}_\sigma$ (defined as before) produces a string of 
	$1$s and $0$s, with the 1s indicating local maxima at scale $\bar{s}=s_\sigma$.
	%----------------------------------------------------
	\item QRE $\qre{oneBL}$ matches one blanking duration, starting with the maximum that initiates it.
	Namely, it matches a maximum (indicated by a~1), followed by a blanking period of length $BL$ samples, followed by any-length string without maxima (indicated by $0^*$):
	$\qre{oneBL} \defeq (1\cdot(0|1)^{BL}\cdot0^*)$
	%----------------------------------------------------
	\item QRE $\qre{latestPeak}$ will return a~1 at the time of the latest peak in the input signal:
	$\qre{latestPeak}=\splitop{right}(\qre{oneBL}^*?0,\,1?1)$.
	It does so by matching all the blanking periods up to this point using $\qre{oneBL}^*$ and ignoring them.
	It then matches the maximum (indicated by~1) at the end of the signal.
	%----------------------------------------------------
	\item QRE $\qre{peakWPB}$ feeds the string of 1s and 0s produced by $\qre{oneMax}_\sigma$ to the QRE $\qre{latestPeak}$:
	$\qre{peakWPB}\,=\,\qre{oneMax}_\sigma\gg \qre{latestPeak}$
\end{itemize}

==> camera - Copy - Copy (2)/chapters/qrepeakWPM.tex <==
\subsection{QRE for WPM}
\label{sec:qre_wpm}
\begin{figure*}[t]
\centering
\includegraphics[scale=0.5]{figures/WPMstream}
\caption{QRE $\qre{peakWPM}$}
\label{fig:WPMstream}
\end{figure*}

A numerical implementation of a CWT returns a discrete set of 
coefficients.
Let $s_1 < s_2 <\ldots <s_n$ be the analysis scales and let 
$t_1,t_2,\ldots$ be the signal sampling times.
Recall that a QRE views its input as a stream of incoming data items.
A data item for WPM is 
$d\,=\,(s_i,\,t_j,\,|\wav(s_i,t_j)|) \in D \defeq (\reals_+)^3$.
We use $d.s$ to refer to the first component of $d$, and $d.|\wav(s,t)|$ to refers to its last component.
The input stream $w\in D^*$ is defined by the values from the spectrogram organized in a column-by-column fashion starting 
from 
the highest scale:
\begin{align*}
\label{eq:fullstream}
w = & \underbrace{(s_n,t_1,|\wav(s_n,t_1)|),\ldots,(s_1, t_1,|\wav(s_1,t_1)|)}_{w_{t_1}}
\ldots
\\
& \ldots
\underbrace{(s_n,t_m,|\wav(s_n,t_m)|),\ldots, (s_1,t_m,|\wav(s_1,t_m)|)}_{w_{t_m}}
\end{align*}
Let $s_\sigma$, $1\leq \sigma\leq n$, the the scale that equals $\bar{s}$.
Since the scales $s_i > s_{\sigma}$ are not relevant for peak detection (their frequency is too low), they should be discarded from $w$.
Now, for each scale $s_{i}$, $i \leq \sigma$, we would like to
find those local maxima of 
$|\wav(s_i,\cdot)|$ that are larger than threshold 
$p_i$\footnote{{\small $p_\sigma = \bar{p}$, $p_{i<\sigma} = 0$,
since we 
threshold only the spectrogram values at scale $\bar{s}$.  After this initial thresholding, tracing of maxima lines returns the peaks.}}. 
We build the QRE $\qre{peakWPM}$ bottom-up as follows. 
In what follows, $i= 1,\ldots,\sigma$.
See Fig.~\ref{fig:WPMstream}.
\begin{itemize}
	\item QRE $\qre{selectCoef}_i$ selects the wavelet coefficient magnitude at scale $s_i$ from the incoming spectrogram 
	column $w_t$.
	It must first wait for the entire colum to arrive in a streaming fashion, so it matches $n$ data items (recall there are $n$ items in a column -- see Fig.~\ref{fig:WPMstream}) and returns as cost $d.|\wav(s_i,t)|$.
	\begin{equation*}
	\qre{selectCoef}_i :=\,(d_nd_{n-1}\ldots d_1?\,d_i.|\wav(s_i,t)|).
	\end{equation*}
	%-----------------------------------------------------------------
    \item \ac{QRE} $\qre{repeatSelectCoef}_i$ applies $\qre{selectCoef}_i$ to the latest column $w_t$.
	To do so, it splits its input stream in two: it executes $\qre{selectCoef}_i$ on the last column, and ignores all columns that preceded it using $(d^n)^*$.
    It returns the selected coefficient $|\wav(s_i,t)|$ from the last column.
    \begin{align*}
    \qre{repeatSelectCoef}_{i} := \splitop{right}((d^n)^*,\, 
    \qre{selectCoef}_i)
    \end{align*}
    Combinator $\splitop{right}$ returns the result of operating on the right-hand side of the split, i.e. the suffix.
%	\begin{align*}
%	repeatSe&lectCoef_{i} \,:=\, \\ 
%	&\splitop{right}(selectCoe\textit{f}\hspace{.4mm}_i^*,\, 
%	selectCoe\textit{f}_i).
%	\end{align*}
%	For instance, figure~\ref{fig:A198WPBs15thr200proj} shows the 
%	output of streaming this QRE on a 
%	spectrogram~\ref{fig:A198WPBs15thr200spec} for a given scale 
%	$s=15$.
	%-----------------------------------------------------------------
	\item QRE $\qre{localMax}_i$ matches a string of real numbers of length at least 3:
	$r_1...r_{k-2}r_{k-1}r_k$.
	It returns the value of $r_{k-1}$ if it is larger than $r_k$ and 
	$r_{k-2}$, and is above some pre-defined threshold $p_i$; 
	otherwise, it returns 0. 
	This will be used to detect local maxima in the spectrogram in a moving-window fashion. In detail: 
	\begin{equation}
	\qre{localMax}_i\,\defeq\,\splitop{right}(\reals^*?0,\,\qre{LM}_3)
	\end{equation} 
	$\qre{localMax}_i$ splits the input string in two: the prefix is matched by $\reals^*$ and is ignored.
	The suffix is matched by QRE $\qre{LM}_3$: $\qre{LM}_3$  matches a length-three string and simply returns $1$ if the 
	middle value is a local maximum that is 
	above $p_i$, and returns zero, otherwise.
	%-----------------------------------------------------------------
	\item QRE $\qre{oneMax}_i$ feeds 
	outputs
	of QRE $\qre{repeatSelectCoef}_{i}$ to the \ac{QRE} $\qre{localMax}_i$.
	\[\qre{oneMax}_i \defeq \qre{repeatSelectCoef}_{i} \gg \qre{localMax}_i\]
	Thus, $\qre{oneMax}_i$ ``sees" a string of coefficient magnitudes $|\wav(s_i,t_1)|,|\wav(s_i,t_2)|,\ldots$ generated by (streaming) $\qre{repeatSelectCoef}_i$, and produces a $1$ at the times of local maxima in this string.
	%-----------------------------------------------------------------
	\item QRE $\qre{peakTimes}_i$ collects the 
	times 
	of local maxima at scale $s_i$ into one set.
	\[\qre{peakTimes}_i\,:=\,\qre{oneMax}_i \gg \qre{unionTimes} \]
	It does so by passing the string of 1s and 0s produced by $\qre{oneMax}_i $ to $\qre{unionTimes}$.
	The latter counts the number of 0s separating the 1s and puts that in a set $\Mc_i$.
	Therefore, after $k$ columns $w_t$ have been seen, set $\Mc_i$ 
	contains all 
	local maxima at scale $s_i$ which are above $p_i$ in those $k$ columns.
	%----------------------------------------------------
	\item QRE $\qre{peakWPM}$ is the final QRE.
	It combines results obtained from scales $s_\sigma$ down to $s_1$:
	\begin{equation*}
	\qre{peakWPM} \,:=\, conn_\delta(\qre{peakTimes}_\sigma,...,\,\qre{peakTimes}_1)
	\end{equation*}
	Operator 
	$conn_\delta$\footnote{{\small Operator $conn_\delta$ can be defined recursively as follows:
	$conn_\delta(X, Y)\,=\,\{y \in Y:\exists x\in X:\, |x-y|\leq \delta\},\,  conn_\delta(X_{k},..,X_1)\,=\,conn_\delta(conn_\delta(X_k,..,X_2),\, X_1)$
%		\begin{align*}
%			&conn_\delta(X, Y)\,=\,\{y \in Y: 
%			\exists x\in X:\, |x-y|\leq \delta\} \\
%			&conn_\delta(X_{k},..,X_1)\,=\,
%			conn_\delta(conn_\delta(X_k,..,X_2),\, X_1)
%		\end{align*}		
	}	} checks if the
		local maxima times for each scale (produced by $\qre{peakTimes}_i$) are within a 
		$\delta$ of the maxima at the previous 
	scale.
\end{itemize}
%=====================================================================
%=====================================================================
In summary, the complete \ac{QRE} is given top-down by:
\begin{align*}
\qre{peakWPM} &\,:=\, conn_\delta(\qre{peakTimes}_\sigma,...,\,\qre{peakTimes}_1)\\
\qre{peakTimes}_i\,&:= \,\qre{oneMax}_i \gg \qre{unionTimes} \\
\qre{oneMax}_i &\defeq \qre{repeatSelectCoef}_{i} \gg \qre{localMax}_i\\
\qre{localMax}_i\,&:=\, \splitop{right}(\reals^*?0,\,\qre{LM}_3) \\
\qre{repeatSelectCoef}_{i} \,&:=\,
\splitop{right}((d^n)^*,\, 
\qre{selectCoef}_i) \\
\qre{selectCoef}_i\,&:=\,(d_n\ldots d_1?\,d.|\wav(s_i,t)|)
\end{align*}

==> camera - Copy - Copy (2)/chapters/related.tex <==
%!TEX root = main.tex

\section{Related Work}
\label{sec:relatedWork}
%Temporal logic~\cite{Pnueli1977} and its extensions~\cite{Maler2004,Donze2012} have gained much success  as concise formal specification languages for expressing temporal behavior. 
Signal Temporal Logic (STL)~\cite{Maler2004} was designed for the specification of temporal, real-time properties over real-valued signals and has been used in many applications including the differentiation of medical signals~\cite{stl-learning,Bartocci2014}. 
In~\cite{BrimDSV14}, STL was augmented with a signal value \emph{freeze operator} that 
 allows one to express oscillatory patterns,
but it is not possible to use it to discriminate
oscillations within a particular frequency range.  
%Furthermore, the associated monitoring algorithm is too complex to be implemented in practice (especially in hardware), since it involves expensive operations over polytopes.
The spectrogram of a signal can be represented as a 2D map (from time and scale to amplitude) and
one may think to employ a spatial-temporal logic such as SpaTeL~\cite{Haghighi2015} or Signal Spatio-Temporal Logic (SSTL)~\cite{Nenzi2015} on spectrograms.
However, both of their underlying spatial models, graph structures for SSTL and quadtrees for SpaTeL, are not appropriate for this purpose.
Logics for describing frequency and temporal properties have been proposed, including
Time-Frequency Logic (TFL) in~\cite{Donze2012} and the approach in~\cite{ChakarovFS2012_TFL}.
TFL is not sufficiently expressive for peak detection 
because it lacks the necessary mechanisms to quantify over variables or to freeze 
their values. 
%Any extension of TFL in this direction would necessarily increase the computational complexity of the generated monitoring algorithm.
Timed regular expressions~\cite{Asarin02_TRE,Ulus16_Montre,UlusFAM14} 
extend regular expressions by clocks and are expressively equivalent 
to timed automata, but cannot express the computations required for 
the tasks covered in this paper. Even the recent work proposed 
in~\cite{FerrereMNU15} on measuring signals with timed patterns is not 
of help in our application, since it does not handle, neither in the specification nor 
in the measurement, the notion of local minima/maxima that is necessary
for peak detection. Furthermore, the operator of measure is separated 
by the specification of the pattern to match.

SRV~\cite{DAngelo2005} is a stream runtime \textit{verification} language that requires explicit encoding of relations between input and output streams, which is an awkward way of encoding the complex tasks of this paper.
Moreover, unlike Boolean SRVs~\cite{Bozzelli2014}, \acp{QRE} allow multiple unrestricted data types in intermediary computations and a number of their questions are decidable for these arbitrary types.

%and Lustre~\cite{CaspiPHP87}, exist, but \acp{QRE} are distinguished by the fact that they allow multiple unrestricted types and the decidability of a number of their questions for any data type.

==> camera - Copy - Copy (2)/chapters/wavelets.tex <==
\subsection{Wavelet Representations}
\label{sec:wavelets}

This definition operates in the wavelet domain, so a brief overview of wavelets is now provided.
Readers familiar with wavelets may choose to skip this section.
%The idea in wavelet analysis is to have a sliding window in which to perform the signal decomposition into its basic components, much like a vector in $\reals^n$ can be decomposed into a weighted sum of basis vectors.
Formally, let $\{\Psi_s\}_{s>0}$ be a family of functions, called \textit{wavelets}, which are obtained by scaling and dilating a so-called \emph{mother wavelet} $\psi(t)$: $\Psi_s(t) = \frac{1}{\sqrt{s}}\psi\left(\frac{t}{s}\right)$.
The \textit{wavelet transform} $\wav$ of signal $\egm: \reals_+ \rightarrow \reals$ is the two-parameter function:
\begin{equation}
\label{eq:cwt}
\wav(s,\,t)=\int\limits_{-\infty}^{+\infty}\,
\egm(\tau)\Psi_s(\tau-t)\,d\tau
\end{equation}
%\vspace{-0.5cm}
An appropriate choice of $\psi$ for peak detection is the $n^{th}$ derivative of a Gaussian, that is: 
$\psi(t) = \frac{d^n}{dt^n}G_{\mu,\sigma}(t)$.
Eq.~\eqref{eq:cwt} is known as a \emph{Continuous Wavelet Transform} (CWT), and $\wav(s,t)$ is known as the \textit{wavelet coefficient.}

Parameter $s$ in the wavelet $\psi_s$ is known as the \emph{scale} of the analysis.
It can be thought of as the analogue of frequency for Fourier analysis.
A smaller value of $s$ (in particular $s<1$) \emph{compresses} the mother wavelet as can be seen from the definition of $\Psi_s$, so that only values close to $\egm(t)$ influence the value of $\wav(s,t)$
(see Eq.~\eqref{eq:cwt}).
Thus, at smaller scales, the wavelet coefficient $\wav(s,t)$ captures \emph{local} variations of $\egm$ around $t$, and these can be thought of as being the higher-frequency variations, i.e., variations that occur over a small amount of time.
At larger scales (in particular $s > 1$), the mother wavelet is \emph{dilated}, so that $\wav(s,t)$ is affected by values of $\egm$ far from $t$ as well.
Thus, at larger scales, the wavelet coefficient captures variations of $\egm$ over large periods of time.

%By performing the wavelet analysis over many scales, we obtain a rich 
%understanding of variations within the signal, the scales at which 
%they occur, and the energy content of such variations. 
Fig.~\ref{fig:nsr and its cwt} shows a Normal Sinus Rhythm EGM and its CWT $|\wav(s,t)|$.
The latter plot is known as a \emph{spectrogram}.
Time $t$ runs along the x-axis and scale $s$ runs along the y-axis.
Brighter colors indicate larger values of coefficient magnitudes $|\wav(s,t)|$.
It is possible to see that early in the signal, mid- to low-frequency content is present (bright colors mid- to top of spectrogram), followed by higher-frequency variation (brighter colors at smaller scales), and near the end of the signal, two frequencies are present: mid-range frequencies (the bright colors near the middle of the spectrogram), and very fast, low amplitude oscillations (the light blue near the bottom-right of the spectrogram).


==> camera - Copy - Copy (2)/chapters/waveletsForPD.tex <==
\section{Peaks in the Wavelet Domain}
\label{sec:peaks in wav domain}

%\vspace{-0.5cm}
Rather than confine ourselves to one particular peak detector, we first describe a general definition of peaks, following the classical work of Mallat and Huang~\cite{MallatH92_Singularity}.
Then two peak detectors based on this definition are presented.
In Section~\ref{sec:experiments}, a third, commercially available, peak detector is also implemented.

\input{chapters/wavelets}

\subsection{Wavelet Characterization of Peaks}
\label{sec:waveletsForPD}
Consider the signal and its CWT 
spectrogram $|\wav(s,t)|$ shown in Fig.~\ref{fig:nsr and its cwt}.
The coefficient magnitude $|\wav(s,t)|$ is a measure of signal power at $(s,t)$.
At larger scales, one obtains an analysis of the low-frequency variations of the signal, which are unlikely to be peaks, as the latter are characterized by a rapid change in signal value.
At smaller scales, one obtains an analysis of high-frequency components of the signal, which will include both peaks and noise.
These remarks can be put on solid mathematical footing \cite[Ch. 6]{waveletMallat}.
\textbf{Therefore, for peak detection one must start by querying CWT coefficients that occur at an appropriately chosen scale $\bar{s}$}.
%Signal variations that occur at scale $\bar{s}$ are indicative of \textit{potential} peaks of interest.

Given the fixed scale $\bar{s}$, the resulting $|\wav(\bar{s},t)|$ is a function of time.
The next task is to find the \emph{local maxima} of $|\wav(\bar{s},t)|$ as $t$ varies.
The times when local maxima occur are precisely the times when the energy of scale-$\bar{s}$ variations is locally concentrated.
\textbf{Thus peak characterization further requires querying the local maxima at $\bar{s}$}.

Not all maxima are equally interesting; rather, only those with  value above a threshold, since these are indicative of signal variations with large energy concentrated at $\bar{s}$.
%Maxima with small value indicate signal variations that, while existing at $\bar{s}$, are better localized on some other scale.
\textbf{Therefore, the specification only considers those local maxima with A value above a threshold $\bar{p}$}. 
%Again, $\bar{p}$ is chosen based on knowledge of the signal class.

Maxima in the wavelet spectrogram are not isolated: as shown in~\cite[Thm. 6.6]{waveletMallat}, when the wavelet $\psi$ is the $n^{th}$ derivative of a Gaussian, the maxima belong to connected curves $s\mapsto \gamma(s)$ that are never interrupted as the scale decreases to~0.
These \emph{maxima lines} can be clearly seen in Fig.~\ref{fig:nsr and its cwt} as being the vertical lines of brighter color extending all the way to the bottom.
Multiple maxima lines may converge to the same point $(0,t_c)$ in the spectrogram as $s\rightarrow 0$.
A celebrated result of Mallat and Hwang~\cite{MallatH92_Singularity} shows that \emph{singularities} in the signal always occur at the convergence times $t_c$.
For our purposes, a singularity is a time when the signal undergoes an abrupt change (specifically, the signal is poorly approximated by an $(n+1)^{th}$-degree polynomial at that change-point). 
\textbf{These convergence times are then the peak times that we seek.} 

Although theoretically, the maxima lines are connected, in practice, signal discretization and numerical errors will cause some interruptions. 
Therefore, rather than require that the maxima lines be connected, we only require them to be $(\epsilon,\delta)$-connected.
Given $\epsilon,\delta>0$, an $(\epsilon,\delta)$-\textit{connected curve} $\gamma(s)$ is one such that for any $s$ in its domain, $|s-s'|<\epsilon \implies |\gamma(s)-\gamma(s')| < \delta$.

A succinct description of this \emph{Wavelet Peaks with Maxima} (WPM) is then:
\let\labelitemi\labelitemii
\begin{itemize}
	\item (Characterization \textit{WPM}) Given positive reals $\bar{s}, \bar{p},\epsilon,\delta >0$, a peak is said to occur at time $t_0$ if there exists a $(\epsilon,\delta)$-connected curve $s \mapsto \gamma(s)$ in the $(s,t)$-plane such that $\gamma(0) = t_0$,  $|\wav(s,\gamma(s))|$ is a local maximum along the $t$-axis for every $s$ in $[0,\bar{s}]$, and $|\wav(\bar{s},\gamma(\bar{s}))|\geq \bar{p} $.
\end{itemize}
The choice of values $\bar{s}$, $\epsilon$, $\delta$ and $\bar{p}$ depends on prior knowledge of the class of signals we are interested in.
Such choices are pervasive and unavoidable in signal processing, as they reflect application domain knowledge.
%Implementations of this characterization can vary in the ways they detect maxima lines $s\mapsto \gamma(s)$, and in their freedom to tighten the degree of connectedness $(\epsilon,\delta)$.
Such a specification is difficult, if not impossible, to express in  temporal and time-frequency logics.
In the next section we show how WPM can be formalized using Quantitative Regular Expressions.

\subsection{Blanking Characterization}
\label{sec:blanking ch}
%\todo[inline]{draw maxima lines, blanking period, etc, on figure.}
For comparison, we modify WPM to obtain a peak characterization that is computationally cheaper but suffers some imprecision in peak-detection times.
We call it \emph{Wavelet Peaks with Blanking} (WPB). 
It says that one peak at the most can occur in a time window of size $BL$ samples.
\begin{itemize}
	\item  (Characterization \textit{WPB}) Given positive reals $\bar{s}$, $\bar{p} >0$, a peak is said to occur at time $t_0$ if $|\wav(\bar{s},t_0)|$ is a local maximum along $t$ and $|\wav(\bar{s},t_0)|>\bar{p}$, and there is no peak occurring anywhere in $(t_0, t_0+BL]$.
\end{itemize}
Section~\ref{sec:experiments} compares WPM and WPB on patient electrograms.
%Note that since this characterization only considers the one scale $\bar{s}$, it may be viewed as essentially a time-domain description. 
%The relationship between WPM and WPB can be established, though we skip the details due to lack of space.
%Let $t_0$ be a peak time found by tracing maxima lines. 
%That is, $(0,t_0)$ is a convergence point for maxima lines. 
%Consider all maxima lines $\{\gamma_i\}$, defined at least on $[0,\bar{s}]$, that converge to $(0,t_0)$ as $s \rightarrow 0$: $\gamma_i(0)= t_0 \; \forall i$.
%Let $C>0$ be a constant s.t.\ for all $i$ and all $s$ in $[0,\bar{s}]$, $(s,\gamma_i(s)) \in \{(s,t) \such |t-t_0|<Cs\}$.
%The latter is known as \emph{the cone of influence} of $\wav(0,t_0)$.
%By choosing $BL = 2C\bar{s}$, the two specifications yield the same number of peaks.
%The difference is that the specification with blanking WPB declares the peak to have occurred at $t_0$ instead of $t_0 + C \bar{s}$ (the center of the cone).
%Moreover, when the heart rate accelerates, more true peaks will fall inside the fixed blanking period and will be ignored, leading to under-detection.


%\begin{theorem}[Mallat Thm. 6.3]
%	\label{thm:uniflip}
%Let $\Psi: \reals \rightarrow \reals$ be a wavelet with $n$ vanishing 
%moments, which is $n$ times continuously differentiable and whose 
%derivatives have fast decay. 
%If $f \in \Lc^2(\reals)$ is uniformly Lipschitz $\alpha \leq n$ over 
%$[a,b]$ then there exists $A > 0$ such that 
%\begin{equation}
%\label{eq:uniflip}
%\forall (s,x) \in \reals^+ \times [a,b], \; |Wf(s,x)| \leq 
%As^{\alpha+1/2}
%\end{equation}
%Conversely, if $Wf(s,x)$ satisfies \eqref{eq:uniflip} and if $\alpha 
%< n$ is not an integer then $f$ is uniformly Lipschitz $\alpha$ on 
%$[a+\epsilon, b-\epsilon]$ for any $\epsilon > 0$.
%\end{theorem}
%Thus if we restrict ourselves to non-integer exponents $\alpha$ over 
%some $[a+\epsilon, b-\epsilon]$, \eqref{eq:uniflip} is a necessary 
%and sufficient condition.
%
%Condition \eqref{eq:uniflip} is really a decay condition on the 
%wavelet transform modulus as $s \rightarrow 0$, since at larger 
%scales the wavelet transform is bounded by the Cauchy-Schwartz 
%inequality ($|Wf(s,x)| = |<f,\Psi_s>| \leq ||f|| \; ||\Psi||$).
%Therefore applying Thm. \ref{thm:uniflip} requires getting the rate 
%of decay of the WT modulus at the finer (smaller) scales.
%
%In practice,the WT is calculated at a finite number of points $x_i 
%\in [a,b]$ and at a finite number of scales $s_i \in \reals^+, 0 \leq 
%i \leq m$.
%Therefore to get the decay exponent, we need to fit a curve $ s 
%\mapsto As^{\alpha+1/2}$ to the data $\{|Wf(s_1,x_i)|, \ldots, 
%|Wf(s_m,x_i)|\}$, for every $x_i$ in $[a,b]$. 
%This yields $A_i,\alpha_i$. 
%The Lipschitz exponent is then the largest of the $\alpha_i$'s.
%
%By re-writing \eqref{eq:uniflip} as
%\[\log |Wf(s,x)| \leq \log(A) + \alpha \log(s)\]
%we can perform a \emph{linear} regression in the log scale.
%The advantage of this expression for our purposes is that the 
%solution of a linear regression is available in closed form.
%Namely, suppose we are given the data $(u_i, y_i)$ and want to fit a 
%line $y = b + \alpha u$. 
%Define the sums
%\[\sigma_c = \Sigma_i c_i \text{ and }  \sigma_{c^2} = \Sigma_i 
%c_i^2, c \in \{u,y, u\cdot y\} \]the best-fit exponent is
%\begin{eqnarray}
%\label{eq:alpha*}
%\alpha^* &=& \frac{\sigma_{uy} - \frac{1}{m+1}\sigma_u 
%\sigma_y}{\sigma_{u^2} - \frac{1}{m+1}\sigma_u^2}
%\\
%b^* &=& \frac{1}{m+1} (\sigma_y - \alpha^* \sigma_u)
%\end{eqnarray}
%The corresponding best fit error is
%\begin{equation}
%\label{eq:delta*}
%\delta^* = \sigma_{y^2} + (\alpha^*)^2 \sigma_{u^2} + (m+1)(b^*)^2 + 
%2b^*\alpha^* \sigma_u - 2\alpha^* \sigma_{uy} - 2b^*\sigma_y
%\end{equation}
%
%Note moreover that it suffices to check \eqref{eq:uniflip} at the 
%local \emph{maxima} of the WT modulus, where the maximum is along the 
%$x$ dimension. 
%That is, we need only consider points $(s',x') \in \reals^+\times 
%[a,b]$ satisfying $|Wf(s',x')| > |Wf(s',x)|$ for all $x$ in either 
%the left or right neighborhood of $x'$, and $|Wf(s',x')| \geq 
%|Wf(s',x)|$ for all $x$ in the other neighborhood.
%As shown in [Mallat Prop. 6.1], when the wavelet is the derivative of 
%a Gaussian, these maxima exist along \emph{connected lines} that are 
%uninterrupted as $s$ goes to 0.
%Thus to reduce computation, it is advantageous to first find these WT 
%modulus maxima (WTMM) lines, and perform the linear regression along 
%these lines.


==> camera - Copy - Copy (2)/chapters/wpbstepstep.tex <==
%WPB RESULTS                                                          
%=====================================================================
\begin{figure}[t]
		\centering
        \includegraphics[width=\linewidth]{figures/A198WPBs15thr200spec}
		\caption{Results of peakWPB running on the PVC signal: 
		Spectrogram of the initial signal}
		\label{fig:A198WPBs15thr200spec}
\end{figure}
%-----------------------------------------------------------------
\begin{figure}[t]
		\centering
		\includegraphics[width=0.92\linewidth]{figures/A198WPBs15thr200proj}
		\caption{Spectrogram 
			projection at the scale $s=15$ with a threshold 
			$\bar{p}=200$}
		\label{fig:A198WPBs15thr200proj}
\end{figure}
%-----------------------------------------------------------------
\begin{figure}[t]
	\centering	
	\includegraphics[width=0.92\linewidth]{figures/A198WPBs15thr200preBL}
	\caption{Results of $preBlank$}
	\label{fig:A198WPBs15thr200preBL}
\end{figure}
%-----------------------------------------------------------------
\begin{figure}[t]
		\centering	
		\includegraphics[width=0.92\linewidth]{figures/A198WPBs15thr200postBL}
		\caption{Results of $peakWPB$ with $BL = 
			100$ ms.}
		\label{fig:A198WPBs15thr200postBL}
\end{figure}
%=====================================================================

Step-by-step results of $peakWPB$ implementation are shown on a 
Figures~\ref{fig:A198WPBs15thr200spec}$-$\ref{fig:A198WPBs15thr200postBL}.
%Such recording correspond to a Premature Ventricular Contraction 
%(PVC) signal. 
%\todo{see figure: should we even go into details about PVC or SVT is 
%enough?}
%\todo{why is PVC signal given as SVT? Is not it always a VT?}
Proper scale projection value setup allows to 
ignore post-event peaks (See Fig.~\ref{fig:A198WPBs15thr200preBL}, 
where high energy peaks around $800$ ms, $2100$ ms, $3050$ ms, and 
$3900$ ms correspond to T waves and, therefore, should not be taken 
into account). 
Blanking period tackles an oversensing problem 
by deleting all additional detected peaks at the cost of the time 
accuracy of detected points, see 
Fig.~\ref{fig:A198WPBs15thr200preBL} and 
\ref{fig:A198WPBs15thr200postBL}. Number of 
detected peaks corresponds to the number of events in the EGM signal, 
but same as before, red circles precede actual peaks.   

==> camera - Copy - Copy (2)/rvPackages.tex <==
% Some macros & packages
% H. Abbass, A. Rodionova - Last update 26.09.2016

\usepackage{fainekos-macros}

\usepackage{makeidx}  % allows for indexgeneration
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{graphicx}
\usepackage{stmaryrd}
\usepackage{tikz}
\usepackage{paralist}
\usepackage{subcaption}
\usetikzlibrary{arrows}
\usepackage{acronym}
%\usepackage[]{todonotes}
% todo notes for the final version - ignores all notes
\usepackage[obeyFinal]{todonotes}
\usepackage{pgfplots}
\usepackage{ifthen}
\usepackage{hyperref} % to create links
\usepackage{mathtools}
\usepackage{balance}
%\usepackage{enumitem}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%\usepackage{oz}
\newcommand\pfun{\mathrel{\ooalign{\hfil$\mapstochar\mkern5mu$\hfil\cr$\to$\cr}}}


% Acronyms
\acrodef{PDA}{Peak Detection Algorithm}
\acrodef{ICD}{Implantable Cardioverter Defibrillator}
\acrodef{QRE}{Quantitative Regular Expression}
\acrodefplural{QREs}{Quantitative Regular Expressions}
\acrodef{RE}{Regular Expression}
\acrodef{EGM}{electrogram}
\acrodef{VF}{Ventricular Fibrillation}
\acrodef{VT}{Ventricular Tachycardia}

% Temporal logic
%\newcommand{\formula}{\varphi}
\newcommand{\qre}[1]{\text{\sf{#1}}}
\newcommand{\freeze}{\downarrow}
\newcommand{\CLTLF}{\text{CLTL}^{\freeze}}
\newcommand{\nxt}{X}
\newcommand{\cmplx}{\mathbb{C}}
% QRE macros
\newcommand{\peakWPM}{peakW\!P\!M}
\newcommand{\peakWPB}{peakW\!P\!B}
\newcommand{\domain}{\mathcal{D}}
\newcommand{\iter}[1]{iter\!-\!#1}
\newcommand{\iterop}{iter\!-\!op}
\newcommand{\iterplus}{iter\!-\!plus}
\newcommand{\splitop}[1]{split\!-\!#1}
\newcommand{\splitp}[1]{\stackrel{[#1\rangle}{\circ}}
\newcommand{\opset}{\mathcal{G}}
\newcommand{\val}[1]{\ensuremath{\llbracket #1 \rrbracket}}

% Signals
\newcommand{\xm}{\underline{x}}
\newcommand{\egm}{x}
\newcommand{\such}{\;|\;}
\newcommand{\wav}{W\!_\egm}
\newcommand{\wavpsi}{W_{\Psi}\!\egm}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,innersep=2pt]
		(char) {#1};}}

==> chapters/algosForPeakDetection.tex <==
\section{Implementing a commercial peak detector as a QRE}
\label{sec:mdt pda}
We now provide a \ac{QRE} implementation of the \ac{PDA} found in some \ac{ICD} models of Medtronic, a major medical devices manufacturer.
This example illustrates two important points about the use of \acp{QRE}:  
the first is that, to target certain applications without violating the constraints of regular parsing, we may need to use a richer set of operations $\opset$ (thus moving some of the complexity of the specification into the operations). 
This is certainly allowed by the current theory of \acp{QRE}, but then one must carefully analyze the resulting evaluation complexity since richer operations will, a priori, require more memory and time. 
In other words, we feel free to enlarge the set of operations without departing from the \ac{QRE} philosophy of being a declarative programming language that allows a global view of the data stream and minimal maintenance of state on the part of the programmer.
The second point this example illustrates is that the streaming setup is useful independently of the basic matching process. 
I.e. whether substreams are matched to regular expressions or, say, bounded temporal logic formulas, the streaming setup and the regular combinators are useful in thinking about the problems we face.

%\begin{figure}[t]
%	\centering
%\includegraphics[scale=0.2]{figures/placeHolder}
%\caption{Peak detection based on a varying threshold as performed in Medtronic devices.}
%\label{fig:mdt pda}
%\end{figure}

\subsection{Natural language description of the peak detector}
The \ac{PDA} defines peaks as points where the signal $y(t) = |\egm(t)|$, which equals the absolute value of the electrogram $\egm(t)$, exceeds a time-varying threshold $p(t)$.
%See Fig. \ref{fig:mdt pda}.
When this happens, a \emph{blanking period} of pre-fixed duration $BL$ is entered. 
In what follows we measure $BL$ in numbers of samples since the sampling rate is uniform.
During the blanking period, no events are recorded, regardless of the relation between threshold and signal.
Also during the blanking period, the maximum value of the signal is recorded.
Let $y(t_m)$ be the value of the maximum, and $t_m$ its time.
At the end of the blanking period, the threshold is reset to the value $0.75 y(t_m)$. 
From there, the threshold decreases exponentially at a pre-specified decay rate $\lambda$.
I.e., after the blanking period, the threshold obeys $p(t) = 0.75y(t_m)e^{-\lambda (t-t_m -BL)}$.
The decay in threshold continues until either a new event is detected, or a minimum threshold value $\underline{p}$ is reached. 
If the minimum threshold value is reached, the threshold remains there until an event is detected.

\subsection{The \ac{QRE}}
\label{sec:mdt pda qre}
The data stream consists of successive uniformly sampled values of $y \in D = \reals$, and the cost domain is $C = \reals$.
The output stream will be a string of time instants when a peak occurred.\footnote{Strictly speaking, the output is a single cost term which is the value of the QRE on the input stream. But stream composition allows us to produce output streams that are then passed along to other QREs.}
If the evolving threshold $p(t)$ were given as part of the input stream\footnote{I.e.. if the data item were $d = (y,p) \in \reals^2$.}, then the above algorithm is easily implemented by concatenating thee QREs: 
the first would iteratively match $y < p$, i.e. $r_1 = (y < p)^*$ ($r_1$ is the RE of the first QRE, etc).
The second would match the signal exceeding the threshold: $r_2 = y \geq p$.
And the third would match the blanking period: $r_3 = D^L$, where $L$ is the blanking duration.
Finally we iterate:
\begin{equation}
r_{mdt1} = (r_1 \cdot r_2 \cdot r_3)^* = ((y<p)^*(y\geq p)D^L)^*
\end{equation}

To produce the time instant at which the peak occurred, the corresponding QRE $mdt1$ only needs to use the sum operation.
Computing the threshold $p$ from the stream $y_1\ldots y_n \in \reals^*$ on the other hand requires a more powerful operation.
The threshold is now treated as a parameter that is updated by the \ac{QRE}. 
Intuitively, with each new voltage value, either the threshold is decreased (in case $y < p$),  or a blanking period is entered (), or a blanking counter is increased (in case $y \geq p$ or the algorithm is already in the blanking period) or the threshold is reset (in case the blanking period expires). 
Because the basic predicates $\phi$ of a symbolic \ac{RE} do not allow to compare a data item $y$ to a parameter value $p$ we need to implement the threshold evolution in an $op$, which we will call $ThEv$.
The implementation details are simple and we omit them for the sake of space.
The peak-detection \ac{QRE} is then simply an iteration of $ThEv$:
\begin{equation}
\label{eq:mdt ThEv}
mdt2 = \iter{ThEv}(d \in \reals?d)
\end{equation}
It is easy to verify that $ThEv$ requires time and memory that are independent of the length of the input string since they only need to consider the current value of the voltage (and internal variables). 
Moreover note that the only basic predicate being used is $d \in \reals$, which takes constant time (in fact, since the data domain is assumed to be $\reals$ no actual check takes place). 
Therefore, despite using a more `powerful' operation, it holds that the evaluator $M_{mdt2}$ processes each data item in time $poly(|mdt2|)$, independently of the length of the string.

\subsection{Experiments}
\label{sec:ex mdt pda}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figures/A177VT2vfiltD1L2Init200BL150}
\caption{\small Rectified EGM of a \ac{VF} showing the peaks detected by QRE $mdt2$ as red circles. By design of this PDA, the circles don't coincide with the actual peaks but precede them by a bit. This doesn't affect the \ac{ICD} operation. }
\label{fig:A177VT2vfiltD1L2Init200BL150}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{figures/A176VT1vfiltD1L2Init300BL80}
	\caption{\small Rectified EGM of a \ac{VT} showing the peaks detected by QRE $mdt2$ as red circles.}
	\label{fig:A176VT1vfiltD1L2Init300BL80}
\end{figure}

We implemented the \ac{QRE} of Eq. \eqref{eq:mdt ThEv}. 
In Fig. \ref{fig:A177VT2vfiltD1L2Init200BL150} we show the results of running it on a \acf{VF} \acf{EGM} collected from a patient during an electrophysiology study.
Note the varying amplitude typical of VF and which is challenging to peak detectors. 
Some peaks are double-counted (e.g. around time 3500) which leads to over-counting and potentially to inappropriate therapy as the heart rate is over-estimated.
Fig. \ref{fig:A176VT1vfiltD1L2Init300BL80} shows $mdt2$ running on a \acf{VT} \ac{EGM}. 
Because \ac{VT} is more organized than a \ac{VF} the \ac{PDA} makes fewer mistakes (in fact, none in this case). 
 
%\input{mdtCLTLformula}

%Given the input string of voltage values, we want to repeatedly extract a substring where the signal is below the threshold (and the threshold is being decreased) followed by a substring where the signal exceeds the threshold (and the blanking period is in effect). 
%I.e. we want to iteratively match the following pattern in the signal:
%\[(y < p? \text{ decrease threshold })^* (y \geq p? \text{ blanking period})\]
%
%First, we describe the threshold decrease. 
%Let $p$ be a parameter holding the value of the threshold, and let $\underline{p} \in \reals$ be the constant that equals the minimum threshold. 
%Then:
%\[decThreshold = iter[p\rangle(y<p? \max(\underline{p}, pe^{-\lambda \Delta t}))\]
%$decThreshold$ matches any strings where the data item $y$ is always below the (decaying) threshold.
%It is of the form QRE($\reals^*, \{p\},\reals$).
%
%Next, the blanking period is conveniently expressed as
%\[blank = (y \geq p?y) \splitp{p} \iter{max}_{BL}(y \in \reals? 0.75y)\]
%This matches a length-$(BL+1)$ string, whose first element exceeds or equals the threshold $p$.
%It evaluates to 0.75 the maximum value of the signal in a window of size $BL$.
%It is of the form QRE($\reals^{BL+1}, \{p\},\reals$).
%
%Since $decThreshold$ and $beat$ are unambiguously concatenatable, we may write
%\[beat = decThreshold \splitp{p} blank\]
%
%Unfortunately, $beat$ is not unambiguously iterable: a string can iteratively match $\reals^*\reals^{BL+1}$ in more than one way.



==> chapters/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We have demonstrated that peak detection, a common and essential signal processing task, cannot be specified in temporal (or time-frequency) logic.
We leveraged a characterization of peaks as singularities in the wavelet domain, formalized it using \acfp{QRE}, and demonstrated its performance on real patient electrograms.
In other work, we use this peak characterization in order to specify various arrhythmia discriminators of ICDs in QREs. 
Finally, it would be very interesting to consider what kind of compile- or run-time analysis questions (e.g., refinement, prediction, and control) can be answered for \acp{QRE} in the specific context of \ac{ICD} verification.


==> chapters/discrimination.tex <==
\section{Arrhythmia Discrimination and Experimental Results}
\label{sec:discrimination}
In Section \ref{sec:many logics} we illustrated the difficulty of using temporal logics 
We briefly illustrate how the discrimination tasks outlined in Section \ref{sec:many logics} can be easily and clearly implemented as QREs.
In this section, we will briefly illustrate how different logics are 
needed for different discriminators, thus prompting the use of 
\acp{QRE}.
%
For example, to
express that the number of heartbeats in a one minute interval must 
be between 90 and 120 requires the usage of a counting modality, such 
as is used
in Counting MTL ($p$ denotes a heartbeat):
\begin{equation*}
	\always \left(start \rightarrow \left(\text{C}_{[120,180]}^{\geq 
		90}p\,\wedge\,\text{C}_{[120,180]}^{< 
		120}p\right)\right)
\end{equation*} 

On the other hand, to express that the heart rate increases by at
least 20\% when measured over consecutive and disjoint windows of 4
beats requires explicit clocks, such as used in XCTL, since the
beat-to-beat delay is variable ($x_i$'s are clocks):
\begin{align*}
	p\,\wedge (x_1=T)\,\wedge\, \eventually(
	p\,&\wedge ...\eventually
	(p\,\wedge\, (x_9=T)\,\wedge\\
	&\wedge\,(x_5-x_1)*0.8 \geq x_9-x_5 )) 
\end{align*}

As a final example, expressing that a threshold $a >0 $ for peak 
detection
is reset as a function of the previous peak value requires us to
remember the value of the peak.  
This necessitates memory registers,
or \emph{freeze quantification} of state variables, such as used in
Constraint LTL with Freeze Quantification $\CLTLF$ ($\freeze$ denotes
the freeze quantifier):
\begin{eqnarray*}
	\always (y > a \implies \freeze_{BL=1} \eventually  \left( 
	\formula_{\text{local-max}} \implies  a = 0.8z_2 \right))
	\\
	\formula_{\text{local-max}} \defeq  \freeze_{z_1=y} \nxt 
	(\freeze_{z_2=y} \nxt (z_2 > z_1 \land z_2> y))
\end{eqnarray*}	
This variety of logics required for these simple tasks, all of which
are fundamental building blocks of ICD operation, means that we
have already lost the unifying view of the entire problem. 

\paragraph{Heart rate}
The average heart rate, averaged over a moving window of size $L$, can be calculated by a QRE.

The QRE $peaks = Lip_{\alpha_0}$ returns a 1 if the the neighborhood it processed had a peak, and 0 otherwise.
If it is fed a string of length which is a multiple of $S \defeq (m+1)(N+1)$, e.g. $\Nc(0:\Delta)\Nc(\Delta:2\Delta)$, we need it to provide an answer only for the last neighborhood.
So we prepend it with a `do nothing' QRE $nothing$ which simply skips a string of length $S$, i.e. we are interested in the QRE $nothing^*peaks$.\footnote{The syntactically correct way of writing this would be as follows: first, $nothing$ is of type QRE$((d\in D)^S,\emptyset,\reals^{|\Xc|})$ where, recall, $\Xc$ is the parameter set of $peaks$.
To skip any prefix whose length is a multiple of $S$ we use $iter[e\rangle (nothing)$ where $e$ is an unused parameter required by the syntax.
Finally to skip such prefix but match the last substream with $peaks$ we simply concatenate:  $heart\!-\!rate = split(iter[e\rangle (nothing) [\Xc\rangle peaks))$. 
Note that $nothing$ is providing the initialization of the parameters in $\Xc$ to $peaks$, which is why we chose its cost domain to be $\reals^{|\Xc|}$.
Note also that $iter[e\rangle (nothing)$ is of type QRE($(D^S)^*, \emptyset, C$) and $peaks$ is of type QRE($D^S, \Xc,\booleans$) so they are unambiguously concatenatable and split is defined for them. 
Moreover, $heart\!-\!rate$ is of type QRE:$((D^S)^*D^S, \emptyset, \booleans)$ so it obeys the typing rules of streaming composition.}

Next If we stream $nothing^*peaks$ (via stream composition) to a sliding window aggregator $\iter{avg}_{[L]}$ , we get the sliding window average of events in the input stream 
\[heart\!-\!rate \defeq nothing^*peaks \gg \iter{avg}_{[L]}\]
(The sliding aggregator computes the average in a window of size $L$ 
\emph{data items}, but because of uniform sampling of the electrogram 
and the fact that all neighbourhoods have the same number of samples, 
a fixed number of data items means a fixed duration for the window.)
The sliding window aggregator ignores null input items $\epsilon$.

\paragraph{Heart rate stability}
The sliding window standard deviation can be similarly computed, and is called the `stability' discriminator as it indicates whether the heart rate is stable (small variance) or unstable (large variance).

\paragraph{Rate comparison}
Given $heart\!-\!rate_A$ and $heart\!-\!rate_V$ which compute the average atrial and ventricular rates respectively, we may compare the two using
\[q_{V>A} = gt(q_{HR,V}, q_{HR, A})\]
where the operation $gt: \reals^2 \rightarrow \booleans$ simply returns True if its first argument is greater than or equal to its second argument, and False otherwise.


==> chapters/formalDefQREsApdx.tex <==
\section{Formal definition of QREs}
\label{formalDefQREs}

For the reviewers' convenience, this appendix gives the formal definition of \acp{QRE}.

For a set $D$ known as the data domain, a \emph{data stream} is a
finite word $w\,{\in}\,D^*$ and a \emph{data language} is a subset
$L\,{\subset}\,D^*$.  Let $\Phi_D$ be a collection of predicates over
$D$ which is closed under the boolean connectives and for which there
exists a finite quantity $time_{\Phi{\rm -}sat}$ such that the
satisfiability of any predicate $\phi\,{\in}\,\Phi_D$ is mechanically
decidable in time less than $time_{\Phi-sat}$.  \emph{Symbolic
  unambiguous regular expressions} (or \acp{RE} for short) are defined recursively as follows:
%
\begin{enumerate}
\item $\epsilon$ is a regular expression and defines the language
  $\val{\epsilon} \defeq \{\epsilon\}$.
\item For each predicate $\phi\,{\in}\,\Phi_D$, $\phi$ is a regular
  expression that identifies the language
  $\val{\phi} \defeq \{d\,{\in}\,D\:{\such}\:\phi(d)\,\text{ holds }\}$.
\item For each pair of regular expressions $r_1, r_2$, if $\val{r_1}$
  and $\val{r_2}$ are disjoint, then $r_1\,{+}\,r_2$ is an \ac{RE} and
  $\val{r_1\,{+}\,r_2}\:{=}\:\val{r_1}\,{\cup}\,\val{r_2}$.
\item For each pair of regular expressions $r_1, r_2$, if $\val{r_1}$
  and $\val{r_2}$ are unambiguously concatenable\footnote{Two
    languages $L_1,L_2\,{\subset}\,D^*$ are unambiguously concatenatable
    if any $w\,{\in}\,L_1L_2$ can be uniquely decomposed into $w=w_1w_2$
    s.t. $w_i\,{\in}\,L_i$.}, then $r_1\,r_2$ is a regular expression and
  $\val{r_1\,r_2} = \val{r_1}\,\val{r_2}$.
\item If $r$ is a regular expression with unambiguously iterable
  language $\val{r}$\footnote{A language $L$ is unambiguously iterable
    if it is non-empty and for any $w\,{\in}\,L^*$ there exists a
    unique decomposition $w = w_1w_2\,{\ldots}\,w_k$
    s.t.~$w_i\,{\in}\,L$ for all $i\,{\leq}\,k$.}, then $r^*$ is an
  \ac{RE} with language $\val{r^*}=\val{r}^*$.
\end{enumerate}

Predicates in $\Phi_D$ are only allowed to examine individual data
values. This restriction guarantees the decidability of questions like
"are two regular expressions disjoint?".  These \acp{RE} will be the
basic way in which patterns are detected in the EGM data.  For
example, given the stream of voltage values $y$,
$(y\,{\leq}\,1)^*(y\,{\geq}\,1)^{200}$ matches any sub-stream that is
below 1, then above 1 for at least 200 samples.

In addition to matching \acf{RE} in the input stream, we need to perform numerical
computations on the sub-streams that match.  A \ac{QRE} augments an
\ac{RE} with \emph{operations} on data types, \emph{parameters} that
are used to pass values between operations, and \emph{regular combinators} that build
more complex \acp{QRE} from simpler \acp{QRE}.  We introduce each 
in turn.
\begin{itemize}
\item Let $\Tc = \{T_1,T_2,\ldots\}$ be a \emph{set of data
  types}. Typical examples include the reals $\reals$, the
  non-negative integers $\Ne$, the booleans $\booleans = \{true,
  false\}$ and  the set $\Me$ of multisets of real numbers.
\item Let $\opset$ be a \emph{set of operations}
  $\{op_1,op_2,\,{\ldots}\}$ on various types, each operation being a
  function of the form
  $op:\,T_1\,{\times}\,{\ldots}\,{\times}\,T_k\:{\rightarrow}\:T$.
  For example, $\opset\:{=}\,\{{+},\,{*},\,{\rm avg},\,x\,{<}\,y\}$ is a set
  of operations on the types $\Tc\,{=}\,\{\reals,\Ne, \booleans\}$.
\item Let $X\,{=}\,(p_1,p_2,\ldots)$ be a \emph{list of parameters}, each
  $p_i$ being of some type $T_i\,{\in}\,\Tc$.
\item A \emph{cost term} $\tau$ is defined using
  $\tau \defeq {p}\:{|}\:{t}\,{\in}\,{T}\:{|}\:op(\tau_1,{\ldots},\tau_k)$
  where $op\,{\in}\,\opset$.  A cost term encodes a mapping
  $\val{\tau}{:}\:{T_1}\,{\times}\,{T_2}\,{\times}{\ldots}{\times}\,{T_k}\:{\rightarrow}\:{T}$
  from parameter valuations $\bar v$ to costs $\val{\tau}(\bar v)$.
\end{itemize}

We denote a valuation of the parameters in $X$ by $\bar v$.  The
valuation $\bar v[p/p_0]$ equals $\bar v$ except at $p\,{\in}\,X$,
where $v_p$ is replaced by $p_0$.

Intuitively, a \ac{QRE} maps a string $w$ to a cost term $f(w)$.  When
a parameter valuation $\bar v$ is given, this then further evaluates
to a cost value in $C$. Formally, for a data domain $D\,{\in}\,\Tc$,
cost domain $C\,{\in}\,\Tc$ and a parameter sequence
$X\,{=}\,(x_1,x_2,{\ldots},x_k)$, a \ac{QRE} $f$ identifies a function
$\val{f}{:}\,D^*\:{\rightarrow}\:({T_1}\,{\times}\,{T_2}\,{\times}\ldots{\times}\,{T_k}\:{\rightarrow}\:{C})\,{\cup}\,\{\bot\}$,
where $\bot$ is the undefined value.

The domain of the \ac{QRE} is the set of strings where it is defined.
Thus each \ac{QRE} is associated with a \acf{RE} $r$ whose language is
the domain of $f$:
$\val{r}\,{=}\,\{w\,{\in}\,D^*\,{\such}\,\val{f}(w)\,{\neq}\,{\bot}\}$.
Following \cite{Alur2016} we write $f$\,{:}\,QRE($r,X,C)$ to indicate
that $f$ is a QRE with RE $r$, parameters $X$ and cost domain $C$.  We
now give the construction rules of \acp{QRE}.  Due to lack of space,
we will only give those constructions that we use in this paper and
refer the reader to \cite{Alur2016} for the full set of constructions.
See Fig.\ref{fig:qre illustrations} for illustrations of the following
definitions.
%
\begin{exmp}
\label{ex:runningApdx}
To illustrate the definitions, we use a simple running example. Let
$\egm{:}\:{\reals_+}\,{\rightarrow}\,\reals$ be a discrete-time signal
(not necessarily uniformly sampled).  The data stream consists of
tuples ${d}\,{=}\,(t,\,{\egm(t)})$ sampled from $\egm$, thus the data
domain is $D\,{=}\,{\reals_+}\,{\times}\,{\reals}$.  Once a \ac{QRE}
is formally defined, from that point onwards, we will occasionally be
less strict about the syntax for the sake of added clarity.
\end{exmp}

\paragraph{\rm\bf 1. Basic functions.}
If $\formula\,{\in}\,\Phi_D$ is a predicate and
$\lambda{:}\,{D}\,{\rightarrow}\,{C}$ is a cost function, then the
semantics of
${\formula}\,{?}\,{\lambda}\,{:}\,\,$QRE($\formula,{\emptyset},{C}$)
is defined as follows:
\[
\val{{\varphi}\,{?}\,{\lambda}}(w,\bar v) = \left \lbrace \begin{matrix}
\lambda(w) &\;& \text{ if }|w|=1 \text{ and } \formula(w) = true,
\\ \bot &\;& \text{ otherwise }
\end{matrix} \right.
\]

\begin{exmp}
Let ${\lambda_1}\,{:}\,(t,\egm(t))\,{\mapsto}\,1$ be the constant 1
function, then the following QRE
$f_1\,{=}\,(d.{\egm}\,{<}\,{-M}\,|\,{d.\egm}\,{>}\,{M})\,{?}\,{\lambda_1}$
matches data items with voltages larger than $M$ in absolute value and
evaluates to 1.  In other words, $f_1$ marks the occurrence of a data
item with $|d.\egm|>M$.  On the other hand,
$f_a\,{=}\,{d}\,{\in}\,{D}\,{?}\,|d.\egm|^2$ maps any item $d$ to the
square of its voltage.
\end{exmp}

\paragraph{\rm\bf 2. Cost operations.}
Operations from $\opset$ can combine the values of individual
\acp{QRE}.  E.g. $sum(f,g)(w,\bar v)$ will produce the value
$\val{f}(w,\bar v)+\val{g}(w,\bar v)$ if both $f$ and $g$ are defined
on $w$ (and will produce $\bot$ otherwise).  Formally, consider an
operation $op\,{\in}\,\opset$ and $f_i\,{:}\,{\rm
  QRE}(r_i,X_i,T_i),~i=1{\ldots}k$.  If the domains are equal
$\val{r_1}\,{=}\,\val{r_2}\,{=}\,\ldots\,{=}\,\val{r_k}$ and the
parameter lists are pair-wise disjoint
$X_i\,{\cap}\,X_j\;{=}\;{\emptyset}$ then
$op(f_1,\ldots,f_k)\,{:}\,{\rm QRE}(r_1, \cup_iX_i, C)$ is defined as
follows:
\[
\val{op(f_1,\ldots,f_k)}(w,\bar v) = \left \lbrace \begin{matrix}
op(\val{f_1}(w,\bar v),\ldots,\val{f_k}(w,\bar v)) &\;& \text{ if }\val{f_i}(w) \neq \bot \forall i
\\
\bot &\;& \text{otherwise}
\end{matrix}\right.\]

\begin{exmp}
Let $\mu$ be a QRE that computes the average of a stream of length
$N$, that is, $\val{\mu}(w,\bar v)\,{=}\,\sum_i w_i.\egm/N$, and
$\sigma_2$ be a QRE that computes the average of the values squared,
that is, $\val{\sigma_2}(w,\bar v)\,{=}\,\sum_iw_i.\egm^2/N$.  Then
the the variance (difference of the two) is computed as $var = {\it
  diff}(\sigma_2, \mu)$.
\end{exmp}

\paragraph{\rm\bf 3. Substitution.}
Let
$f\,{:}\,{\rm QRE}(r_f,X_f,T_f)$ and $g\,{:}\,{\rm QRE}(r_g,X_g,T_g)$
be a pair of \acp{QRE} with equal domain $\val{r_f} = \val{r_g}$ and let the parameter $x \in X_f$ of type $T_g$ be the only shared parameter between $X_f$ and $X_g$.
Informally, the expression $f[x/g]$ substitutes the result of applying $g$ on $w$ for $x$, before evaluating $f$.
Formally, if both $\val{f}(w)$ and $\val{g}(w)$ are defined
$\val{f[x/g]}(w,\bar v) = \val{f}(w, \bar v[x/int_g])$ where $int_g = \val{g}(w,\bar v)$.
Otherwise it is undefined.

\paragraph{\rm\bf 4. Conditional choice.}
If we wish to also mark the occurrence of absolute voltage values
smaller than $M$, then we can use a conditional as follows:
\[
f_{01}\defeq (f_1 \; {\rm else} \; \underbrace{(d.\egm > -M \;\land \; d.\egm
  <M)\,{?}\,\lambda_0}_{f_0})
\]
where $\lambda_0$ is the constant 0 function.  This accepts a data
item and outputs 1 if $|d.\egm| > M$ (via $f_1$), else it outputs 0 (via $f_0$).
Formally, if $f$ and $g$ are \acp{QRE} with disjoint domains then
$f\;{\it else}\;{g}\,{:}\,{\rm QRE}(r_f\,{+}\,r_g, X_f\,{\cup}\,{X_g},
T_f\,{\cup}\,{T_g}$) and is given by
\[
\val{f\;{\it else}\;g}(w,\bar v) = \left \lbrace \begin{matrix}
int_f &\;& \text{ if }int_f \neq \bot, \text{ and } 
\\
\val{g}(w,\bar v) &\;& \text{ otherwise }
\end{matrix} \right.
\]
with $int_f = \val{f}(w,\bar v)$ is the semantics of QRE $f$.

\paragraph{\rm\bf 5. Concatenation.}
While a cost operation combines costs of \acp{QRE} that match the same
input stream, a concatenation combines costs of \acp{QRE} that match
disjoint \emph{substreams} of the input stream.  We now define a
restricted version of concatenation that we use in this paper.  A more
general concatenation combinator is defined in \cite{Alur2016}.  Let
$f\,{:}\,{\rm QRE}(r_f,X_f,T_f)$ and $g\,{:}\,{\rm QRE}(r_g,X_g,T_g)$
be a pair of \acp{QRE} with unambiguously concatenatable domains and
such that $X_f\,{\cap}\,X_g\;{=}\,{\emptyset}$. 
Let $op\,{\in}\,\opset$ be a binary operation.  Then
$\splitop{op}(f,g)$ is a QRE of the form ${\rm QRE}(r_fr_g,
X_f\,{\cup}\,X_g, T_g)$.  If an input stream $w$ can be uniquely split
into $w\,{=}\,w_f w_g$ such that both $\val{f}(w_f)$ and
$\val{g}(w_g)$ are defined then
$\val{\splitop{op}(f,g)}(w)\,{=}\,op(\val{f}(w_f), \val{g}(w_g))$.
Otherwise it is undefined.

\begin{exmp}
Consider the operation $gt$ defined by $gt(x,y)\,{=}\,x\,{>}\,y$ which
evaluates to $true$ if $x\,{>}\,y$.  Then
$split-gt(d\,{\in}\,D\,{?}\,d.\egm, d\,{\in}\,D\,{?}\,d.\egm)$ splits
a stream of length two and returns the value true if the first
element's voltage is greater than the second element's voltage.
\end{exmp}

\paragraph{\rm\bf 6. Iteration.}

The analog of the Kleene's star operator $(\_)^*$ on regular
expressions is iteration.  Consider $f\,{:}\,{\rm QRE}(r,X,T)$ with
unambiguously iterable domain and $p$ a parameter of type $T$.  Then
$f^*\,{=}\,iter[p\rangle(f)$ is a \ac{QRE} of the form
${\rm QRE}(r^*, \{p\}, T)$. It is defined on the input stream $w$ if
the latter can be uniquely divided into $w=w_1w_2{\ldots}w_k$ such
that $\val{f}(w_i)$ is defined for every $i$.  Intuitively, $f^*$ will
first evaluate $f$ on $w_1$: $int_1\,{=}\,\val{f}(w_1,\bar v)$.  This
intermediate value is passed to the next iteration which computes
$int_2\,{=}\,\val{f}(w_2,\bar v[x/int_1])$.  And so on up to $k$.  Thus
each iteration passes its output to the next iteration which can use it.

%The second intermediate value is passed along to the third
%evaluation as a parameter, and so on up to $k$.
%
%Intuitively, $f^*$ evaluates $f$ on each substream $w_i$.  When
%evaluating $\val{f}(w_i)$, it uses the output of the previous
%evaluation (namely, $\val{f}(w_{i-1})$ to initialize the value of
%parameter $p$ in the current evaluation .  Thus $p$ serves to set the
%context for from one iteration to the next.

See Fig. \ref{fig:qre illustrations} for a graphical illustration
of iteration.  Formally, given a valuation
$\bar v$, the intermediate values $int_i$ are defined as follows:

\begin{itemize}
\item {\it Initialization:} $int_0 = v_p$, the value of $p$ under the valuation $\bar v$.
\item {\it Iteration:} $int_i = \val{f}(w, \bar v[p/int_{i-1}])$.
\item {\it Termination:} $\val{iter[x\rangle(f)}(w,\bar v) = int_k$.
\end{itemize}

It can be shown that this iterator can implement \acp{QRE} of type
$\iterop(f)$, where at each iteration, the value $op(int_{i-1},
\val{f}(w_i))$ is computed.  For example, sum, average, max, min,
etc.,~of a stream of numbers, is easily implemented.

\begin{exmp}
Say we want to count the number of data items whose absolute voltage
exceeds threshold $M$.  Then we are interested in $\iter{sum}(f_0)$,
which accepts a stream of values below the threshold and outputs 0
(recall that every match of $f_0$ produces a 0, thus their sum is 0).
We also need to iterate $\iter{sum}(f_1)$, which will match
$(|d.\egm|\,{>}\,{M})^*$ and output the length of the matching stream.
We then concatenate the two: $\iter{sum}(f_0)\cdot \iter{sum}(f_1)$
will match $(|d.\egm|\,{\leq}\,M)^*(|d.\egm|\,{>}\,M)^*$ and output
the number of times the threshold was exceeded.  Finally, we iterate
that last QRE over the entire stream.
\end{exmp}

\paragraph{\rm\bf 7. Stream composition.}
Very often we are interested in generating intermediate streams $z \in
C^*$ from the data stream $w \in D^*$.  These can then be further
processed by other \acp{QRE} to produce a final cost term. In our
running exmaple, $f_{01}$ can produce a stream of 0s and 1s which is
further processed.  Streaming composition achieves this.  Let
$f\,{:}\,{\rm QRE}(r_f,\emptyset,T_f)$ and $g\,{:}\,{\rm
  QRE}(T_f^*,X_g,T_g)$ be a pair of \acp{QRE}.  Note that $g$ is
defined over all intermediate data streams produced by $f$.  Then
$f\,{\gg}\,{g}\,{:}\,{\rm QRE}(D^*,X_g,T_g)$.  Given the input stream
$w=w_1w_2{\ldots}w_k$ and parameter valuation $\bar v$, define the
intermediate results $int_i$, $i\,{\leq}\,k$, as follows:

\begin{itemize}
\item {\it If}\;\;$\val{f}(w_1w_2{\ldots}w_i, \bar v)\,{\neq}\,\bot$ then
  $int_i\,{=}\,\val{f}(w_1w_2{\ldots}w_i, \bar v_{\emptyset})$ where
  $\bar v_{\emptyset}$ is the empty parameter valuations.
\item {\it Otherwise} $int_i =\epsilon$.
\item {\it Finally} $\val{f \gg g}(w,\bar v) = \val{g}(int_1 int_2 \ldots int_k, \bar v)$.
\end{itemize} 


%QREs do place some restrictions on the basic predicates and how costs are 
%combined. 
%Most notably, 
%These will be reviewed later, and are motivated by the desire to 
%maintain decidability of fundamental questions like: are two REs 
%equivalent? and to obtain reasonable complexity for computing the 
%value of a QRE.
%Because our concerns in this paper are mainly about the performance 
%of runtime monitoring, we will feel free to relax some of the 
%restrictions that are mainly motivated by decidability questions, 
%without straying far from the QRE philosophy.


==> chapters/fourierBlurb.tex <==
\begin{figure}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{figures/sin_fft}
	\caption{Signal of Fig.~\ref{fig:sin_signal} in Fourier domain}
	\label{fig:sin_fft}
\end{figure}
To analyze the properties of a stationary signal $\egm: \reals_+ \rightarrow \reals$, it is convenient to decompose it into its harmonics, which are sinusoids with a particular phase and frequency. 
Since $e^{iwt} = \cos wt + i\sin wt$, the signal can equivalently be decomposed into a sum of complex exponentials.
This is accomplished through the use of the \emph{Fourier Transform}~\cite{waveletMallat}: 
%% ($i=\sqrt{-1}$)
\begin{equation}
\label{eq:fourier pair}
\hat{\egm}(w)=\int\limits_{-\infty}^{+\infty}\egm(t)e^{-iwt}\,dt,
\qquad
\egm(t)=\frac{1}{2\pi}\int\limits_{-\infty}^{+\infty}\hat{\egm}(w)
e^{iwt}\,dw
\end{equation}
$\hat{\egm}(w)$ is called the Fourier transform of $\egm(t)$.
Eq.~\eqref{eq:fourier pair} proves that the transform is invertible and so the signal is uniquely determined by either its time-domain or Fourier-domain description.
Parameter $w$ is the frequency: $|\hat{\egm}(w)|$ gives the power of the signal at frequency $w$. 
Thus, the larger $|\hat{\egm}(w)|$, the more energy is contained at that frequency. 

For example, the signal $\egm(t)$ in Fig.~\ref{fig:sin_signal} 
contains three distinct regimes of variation at different 
frequencies.
The first regime contains two periods of a slow (5Hz frequency) sinusoid, the second contains fifteen periods of fast (10 Hz) sinusoid, and the third contains the superposition (linear composition) of the first with a very fast (35 Hz) sinusoid. 
The fast harmonics in the last regime can be thought of as constituting noise. 
The Fourier transform of $\egm(t)$ is depicted in
Fig.~\ref{fig:sin_fft} and shows three large components at the 
frequencies 5, 10 and 35 Hz.
The frequency domain provides a very intuitive way of capturing the harmonics of a signal, and the Fourier Transform is a tool for bringing these harmonics to light. 
In contrast, writing a temporal formula capturing a signal of one or several frequencies is impractical.

The Fourier transform gives the frequency content, but \emph{does not localize it in time}. 
Looking at Fig.~\ref{fig:sin_fft}, one cannot further specify whether the 35 Hz component occurs early or late in the signal.
A solution would be to take a Fourier transform in a sliding window of the signal, but this raises questions of which windowing function to use, how wide it should be, the amount of overlap between windows, etc.

==> chapters/wpbstepstep.tex <==
%WPB RESULTS                                                          
%=====================================================================
\begin{figure}[t]
		\centering
        \includegraphics[width=\linewidth]{figures/A198WPBs15thr200spec}
		\caption{Results of peakWPB running on the PVC signal: 
		Spectrogram of the initial signal}
		\label{fig:A198WPBs15thr200spec}
\end{figure}
%-----------------------------------------------------------------
\begin{figure}[t]
		\centering
		\includegraphics[width=0.92\linewidth]{figures/A198WPBs15thr200proj}
		\caption{Spectrogram 
			projection at the scale $s=15$ with a threshold 
			$\bar{p}=200$}
		\label{fig:A198WPBs15thr200proj}
\end{figure}
%-----------------------------------------------------------------
\begin{figure}[t]
	\centering	
	\includegraphics[width=0.92\linewidth]{figures/A198WPBs15thr200preBL}
	\caption{Results of $preBlank$}
	\label{fig:A198WPBs15thr200preBL}
\end{figure}
%-----------------------------------------------------------------
\begin{figure}[t]
		\centering	
		\includegraphics[width=0.92\linewidth]{figures/A198WPBs15thr200postBL}
		\caption{Results of $peakWPB$ with $BL = 
			100$ ms.}
		\label{fig:A198WPBs15thr200postBL}
\end{figure}
%=====================================================================

Step-by-step results of $peakWPB$ implementation are shown on a 
Figures~\ref{fig:A198WPBs15thr200spec}$-$\ref{fig:A198WPBs15thr200postBL}.
%Such recording correspond to a Premature Ventricular Contraction 
%(PVC) signal. 
%\todo{see figure: should we even go into details about PVC or SVT is 
%enough?}
%\todo{why is PVC signal given as SVT? Is not it always a VT?}
Proper scale projection value setup allows to 
ignore post-event peaks (See Fig.~\ref{fig:A198WPBs15thr200preBL}, 
where high energy peaks around $800$ ms, $2100$ ms, $3050$ ms, and 
$3900$ ms correspond to T waves and, therefore, should not be taken 
into account). 
Blanking period tackles an oversensing problem 
by deleting all additional detected peaks at the cost of the time 
accuracy of detected points, see 
Fig.~\ref{fig:A198WPBs15thr200preBL} and 
\ref{fig:A198WPBs15thr200postBL}. Number of 
detected peaks corresponds to the number of events in the EGM signal, 
but same as before, red circles precede actual peaks.   
